Beyond Deepfake Images: Detecting AI-Generated Videos

Recent advances in generative AI have led to the development of techniques to generate visually realistic synthetic video. While a number of techniques have been developed to detect AI-generated synthetic images, in this paper we show that synthetic image detectors are unable to detect synthetic videos. We demonstrate that this is because synthetic video generators introduce substantially different traces than those left by image generators. Despite this, we show that synthetic video traces can be learned, and used to perform reliable synthetic video detection or generator source attribution even after H.264 re-compression. Furthermore, we demonstrate that while detecting videos from new generators through zero-shot transferability is challenging, accurate detection of videos from a new generator can be achieved through few-shot learning.

==> figures/crf_plot.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/crf_AUC_plot.png}
    \caption{Performance plot of of Mislnet trained on different synthetic video generation methods: Luma~\citethis, CogVideo~\citethis, VideoCrafter (VC-v1)~\citethis, and Stable Video Diffusion (SVD)~\citethis. Performance numbers are measured using AUC. The baseline plot demonstrates the performance of detector for each CRF without robust training and the average plot demonstrate the average performance over four generators after robust training}
    \label{fig:crf_auc_plot}
\end{figure}

==> figures/figure1.tex <==
\begin{figure*}[!h]
	\centering
	\setlength{\fboxsep}{0pt}
	\begin{minipage}[t]{1.0\textwidth}
		\centering
		\setlength{\fboxrule}{-1pt}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller ProGAN}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Latent Diffusion}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller CycleGAN}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller StarGAN}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller StyleGAN 3}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Stable Image Diffusion}}
		\smallskip
	\end{minipage}
	
	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-1pt}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/progan}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/luisa}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/cyclegan}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/stargan}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/stylegan3}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/stable_img}}}
	\end{minipage}
	
	\begin{minipage}[t]{1.0\textwidth}
		\centering
		\setlength{\fboxrule}{-1pt}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Luma}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller VideoCrafter}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller CogVideo}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Pika}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Sora}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Stable Video Diffusion}}
		\smallskip
	\end{minipage}
	
	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{-1pt}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/luma}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/vidcrafter}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/cogvideo}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/pika}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/sora}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/final_vis/stable_video}}}
	\end{minipage}
	
	\caption{hey}
	\label{fig:front_page_graphics}
\end{figure*}

==> figures/trace_vis_v0.tex <==
\begin{figure*}[!h]
	\centering
	\setlength{\fboxsep}{1pt}
	\begin{minipage}[t]{1.0\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
        \setlength{\fboxsep}{0pt}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller ProGAN}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Latent Diffusion}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller CycleGAN}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller StarGAN}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller StyleGAN 3}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Stable Image Diffusion}}
		\smallskip
	\end{minipage}
	
	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/progan}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/latent_diffusion}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/cyclegan}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/stargan}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/stylegan3}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/stable_img}}}
	\end{minipage}
	
	\begin{minipage}[t]{1.0\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Luma}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller VideoCrafter}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller CogVideo}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Pika}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Sora}}
		\fbox{\parbox{0.150\textwidth}{\centering\smaller Stable Video Diffusion}}
		\smallskip
	\end{minipage}
	
	\begin{minipage}[t]{1\textwidth}
		\centering
		\setlength{\fboxrule}{0pt}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/luma}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/videocrafter}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/cogvid}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/pika}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/sora}}}
		\fbox{\includegraphics[width=0.150\textwidth]{{figures/trace_visualization/stable_vid}}}
	\end{minipage}
	
	\caption{Fourier transform analysis of the forensic traces extracted from different synthetic image and video generators. Top row shows the synthetic image traces: from left to right ProGAN~\cite{progan}, Latent Diffusion~\cite{diffusion7}, CycleGAN~\cite{cyclegan}, StarGAN~\cite{stargan}, StyleGAN 3~\cite{stylegan3}, and Stable Image Diffusion~\cite{stablediffusion} Bottom row shows the synthetic video traces: from left to right Luma~\cite{Luma}, VideoCrafter~\cite{videocrafter1}, CogVideo~\cite{cogvideo}, Pika~\cite{Pika}, Sora ~\cite{sora}, and Stable Video Diffusion~\cite{stablevideo}}
	\label{fig:trace_visualization}
\end{figure*}

==> figures/video_auc.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/video_level.png}
    \caption{Video-level performance of MISLnet\citethis over different number of patches trained on four video generators before and after robust-training with CRF-40 r-ecompressed video frames. Performance is measured in AUC.}
    \label{fig:crf_auc_plot}
\end{figure}

==> figures/video_rer.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{figures/RER_plot.png}
    \caption{Video-level performance of MISLnet\citethis over different number of patches trained on four video generators before and after robust-training with CRF-40 r-ecompressed video frames. Performance is measured in RER.}
    \label{fig:crf_auc_plot}
\end{figure}

==> sec/Abstract_v0.tex <==
\begin{abstract}
\textbf{ABSTRACT MADE USING CHATGPT - NEEDS REVISING}
Detecting synthetic images generated by diverse and evolving techniques is crucial for combating misinformation and disinformation. Existing approaches face challenges in adapting to new generators due to limited data availability and the risk of catastrophic forgetting. In this paper, we propose an Ensemble of Expert Embedders (E3) framework to address these challenges. E3 employs specialized embedders, created via transfer learning, to capture traces from specific generators. These embedders' outputs are analyzed by an Expert Knowledge Fusion Network (EKFN) to enhance detection accuracy. Experimental results demonstrate that E3 outperforms existing methods, offering superior adaptability to new generators while mitigating traditional challenges. E3 presents a novel and effective approach for continually updating synthetic image detectors in response to emerging generation techniques.
    
\end{abstract}

%Recent advancements in generative artificial intelligence have enabled the creation of highly realistic synthetic images and videos, exacerbating the threat of misinformation and disinformation. While considerable progress has been made in developing techniques to detect synthetic images by identifying generator-specific statistical traces, the emergence of synthetic video generators poses new challenges. This paper investigates the effectiveness of existing synthetic image detection techniques when applied to synthetic videos and reveals a significant performance gap. We demonstrate that synthetic video generators leave behind unique traces that differ substantially from those found in synthetic images, which current detectors are not trained to identify. Our findings show that while traditional synthetic image detectors struggle to accurately detect synthetic videos, they can be trained to learn these unique traces, enabling reliable detection and generator source attribution. Moreover, we explore the transferability of these detectors to identify content from previously unseen generators, finding that few-shot transferability is achievable with minimal fine-tuning. To support further research, we introduce a novel dataset of synthetic videos generated by a variety of methods. Our contributions highlight the need for specialized detection techniques for synthetic videos to combat the evolving threat of AI-generated disinformation.

==> sec/Abstract_v1_DSV.tex <==
\begin{abstract}
    Recent advancements in generative artificial intelligence have led to highly realistic synthetic images and videos, escalating the threat of misinformation. While progress has been made in detecting synthetic images by identifying generator-specific statistical traces, the emergence of synthetic video generators presents new challenges. This paper investigates the effectiveness of using synthetic image detectors in detecting synthetic videos and reveals a significant performance gap. We demonstrate that synthetic video generators leave unique traces that differ from those in synthetic images, posing challenges for current detectors. However, detectors can be trained to reliably detect synthetic videos and attribute them to their source generators.We also explore the transferability of these detectors to identify content from new generators, finding promising results with few-shot learning. Additionally, we introduce a dataset of synthetic videos to support further research. Our findings underscore the necessity for specialized detection techniques to combat AI-generated disinformation effectively.
\end{abstract}

==> sec/Exp2_SynthVidAttr_v4.tex <==



\subsection{Synthetic Video Source Attribution}
\label{subsec:exp2_synth_vid_attr}

Next, we conducted an experiment in which we evaluated each  network's ability to perform source attribution.  In this scenario, the forensic network must identify a video's source generator (or determine that the video is real). To adapt each network for this multi-class classification problem, we replaced its final layer with one containing multiple neurons, one for each generator along with an additional neuron for real.  Each network was trained to minimize the cross entropy between its soft-maxed output and a one hot vector identifying the true video source.  The trained network's AUC was assessed using the one-vs-the-rest strategy, i.e. any incorrect source attribution was counted as a miss irrespective of the class.

\input{tables/exp2_synth_vid_attr_v0}

The results of this experiment are shown in Table \ref{tab:exp2_synth_vid_attr}.  From these results, we can see that 
all networks achieved an AUC of at least 0.91, with most achieving an AUC of 0.95 or higher.  Again, the best performing network was MISLnet, which acheived an AUC of 0.991.
These results indicate that existing networks can be trained to perform accurate synthetic video source attribution.  We note that this result makes sense in light of the synthetic video traces visualized in Fig.~\ref{fig:trace_visualization}.  As discussed in Sec.~\ref{sec:synth_video_traces}, videos are generated using a wide variety of generation strategies and generator architectures.  As a result, there are often significant differenes between the traces left by each generator.  This makes it much easier for networks to accurately discriminate between each generator.




==> sec/Exp3_Recompression_v4.tex <==



\subsection{Effect of H.264 Re-compression}
\label{subsec:exp3_vid_compression}

\input{figures/exp3_recompression}

As we discussed in Sec.~\ref{sec:synth_img_det_on_videos}, it is well known that re-compression can significantly reduce the performance of a forensic system.  
%
This is particularly important since re-compression is often utilized by social media platforms.  
%
In light of this, we conducted a set of experiments to understand the effect of H.264 compression on detection performance.  Additionally, we conducted experiments to assess the ability of robust training to mitigate these effects.
In light of space constraints, results are reported for the MISLnet detector, which achieved the highest detection and attribution performance in the previous experiments.

To carry out these experiments, we re-compressed each video in the testing set with constant rate factors (CRFs) ranging from 0 (weak) to 40 (strong) in increments of 10. We note that videos are all initially H.264 compressed by either the camera that captured them or the system that generated them. 
Typically, this is done using a default CRF of 23 or similar value. 
We then re-compressed each video in the training set using the same CRF levels, then robustly trained MISLnet to perform synthetic video detection using this data.
After this, we evaluated the performance of both the non-robustly trained and robustly trained version of this detector.

The results of this experiment are displayed in Fig.~\ref{fig:exp3_recompression}, which shows the AUC achieved by the detector at each CRF both with and without robust training.  
% 
From these results, we can see that without robust training, the detector's performance decreases as the CRF increases.  The notable exception to this is at CRF 20, which is close to the typical default CRF of 23.  Performance increases here because the CRF used during re-compression is close to the default CRF that has already been seen during training.  

The results presented in Fig.~\ref{fig:exp3_recompression} also show that when robust training is utilized, the detector's performance remains consistently strong across all CRFs.
Specifically, the detector is able to achieve an AUC of 0.95 or higher for all CRFs.  Furthermore, when the CRF is greater than or equal to 30, the detector is able to achieve an AUC of 0.97 or higher.  These results show that robust training can enable accurate synthetic video detection even after a video has been re-compressed.


















==> sec/ExpSetupVid_v4.tex <==
\subsection{Experimental Setup}
\label{subsec:common_video_exp_setup}

\input{tables/video_dataset_stats_v1}

The following experiments all used the same experimental setup detailed here. 

\subheader{Video Training Data}
To train synthetic video detection systems in the following experiments, we collected a diverse set of real and synthetic videos. 

For the set of real videos, we gathered videos from both the Moments in Time (MIT)~\cite{mit} dataset and the Video-ACID~\cite{videoacid} dataset. Videos in the MIT dataset have much greater scene and content diversity, while videos in the Video-ACID dataset have much higher resolution and all videos came directly from video cameras. 

For the set of synthetic videos, we used 4 publicly available video generators to generate a large dataset for both training and testing purposes. These generation methods are: Luma~\cite{Luma}, VideoCrafter-v1~\cite{videocrafter1}, CogVideo~\cite{cogvideo}, and Stable Video Diffusion~\cite{stablevideo}. 
To create the synthetic videos in our dataset, we utilized a common set of text prompts chosen to represent a diverse set of motions and scenes.  Videos created using Luma were gathered from publicly shared videos, and similarly chosen to represent a diverse set of contents and activities. 

Additionally, we note that all videos is by default compressed using H.264 at CRF 23 since raw video is essentially never produced by a camera or a generator. More detailed are provided in Tab.~\ref{tab:video_dataset_stats}.

\subheader{Video Testing Data}
To form the set of testing videos used in the following experiments, we utilized the same collection and generation methodology as for our training data. However, we kept an exclusive set of testing prompts to only be used to create testing data. Regarding videos from Luma, we also gathered a disjoint set of videos, completely separate from those in the training set. We note that this testing set is the same testing set used for experiments in Sec.~\ref{sec:synth_img_det_on_videos}. More detailed are provided in Tab.~\ref{tab:video_dataset_stats}.


\subheader{Out-of-distribution Test-only Synthetic Videos}
In addition to our in-distribution video testing set, we also evaluated the performance of different detection algorithms on an out-of-distribution, test-only set of videos. The synthetic videos in this set is collected from three recently emerging generation methods: Sora~\cite{sora}, Pika~\cite{Pika}, and VideoCrafter-v2~\cite{videocrafter2}. More details on this dataset are provided in Tab.~\ref{tab:ood_dataset_stats}

\subheader{Metrics}
In the following experiments, the performance of each detector was measured using the area under its ROC curve (AUC). In addition, to highlight performance differences, we provided the Relative Error Reduction (RER) with respect to the second best performing method, reported as a percentage. This metric is calculated as follows:
\skipless
\begin{equation}
	RER = 100 \times \frac{\text{AUC}_{N} - \text{AUC}_{R}}{1 - \text{AUC}_{R}}, 
\end{equation}
where $\text{AUC}_{R}$ is the AUC of the referencing method, and $\text{AUC}_{N}$ is the AUC of the method being compared against.

\skipnormal


\subheader{Detectors}
To demonstrate the performance of different detection methods on detecting synthetic videos, we conducted our experiments with the diverse set of detectors listed in Sec.~\ref{subsec:synth_img_exp_setup} and in Tab.~\ref{tab:list_of_detectors}.






==> sec/FewShotTransfer_v3_DSV.tex <==



\subsection{Experiment 2: Few-shot Learning for Emerging Generation Sources}
\label{subsec:exp_few_shot}

\input{tables/table_few_shot}

In this section, we investigate how few-shot learning can be used to adapt an existing pretrained detector to detect emerging video generation sources. To do this, we first took MISLnet~\cite{bayar2016deep,openset}, the best performing architecture in prior experiments in our paper, and trained this network architecture on the entire set of real and synthetic training videos in our dataset (described in Sec.~\ref{subsec:common_exp_setup}). Then, we tested this network on three new and emerging video generation sources: Sora~\cite{sora}, Pika~\cite{Pika}, and VideoCrafter v2~\cite{videocrafter2} to get a zero-shot transference baseline. And finally, we applied few-shot learning over this system and evaluate its few-shot performance over each sources.
Specifically, we performed few-shot learning by fine-tuning the pre-trained detector using only 50 seconds of video from each generation sources and tested on 5,000 video frames from Sora\cite{sora}, 10,000 video frames from Pika\cite{Pika}, and 10,000 video frames from VideoCrafter v2\cite{videocrafter2}.
We reported the results of this experiment in Tab.~\ref{tab:few_shot_learning}.

Tab.~\ref{tab:few_shot_learning}'s results show that MISLnet\cite{bayar2016deep,openset} achieved low amount of zero-shot transference on Sora~\cite{sora}, some level of zero-shot transference on Pika~\cite{Pika}, and high level of transference on VideoCrafter v2~\cite{videocrafter2}. However, when this network is allowed to see only 50 seconds of video from each generation source, MISLnet\cite{bayar2016deep,openset} displayed strong detection performance across all sources. This suggests that few-shot learning can be leveraged to address the challenge of detecting novel synthetic videos made using new generation techniques. 

==> sec/FewShotTransfer_v4_MCS.tex <==


%\subsection{Experiment 2: Few-shot Learning for Emerging Generation Sources}
%\subsection{Few-Shot Transferabilty}
\subsection{Transferabilty Through Few-Shot Learning}
\label{subsec:exp_few_shot}


\input{tables/table_few_shot_v1_DSV}

%Next, we examined the ability of synthetic video detectors to transfer to new generators through few-shot learning. 

Next, we examined the ability of a synthetic video detector to transfer detect a new generator through few-shot learning. 

%Next, we conducted a experiments to examine the ability of synthetic video detectors to achieve few-shot transferability, i.e. its ability to detect videos from a new generator given a limited amount of training data.



%To conduct these experiments, we fine-tuned our pre-trained detector% using the MISLnet-architecture

To conduct these experiments, we started with a detector that was pre-trained to detect all four generators in the training set.  As in the previous experiment, we used MISLnet for our detector.   Next, we fine-tuned the detector to detect each generator in the Out-of-Distribution testing set using less than one minute of video from each generator.  We note the video used for fine-tuning was not included in the testing set.  After updating the detector, we measured its its ability to detect each new generator in the Out-of-Distribution testing set.

Results of this experiment are shown in the right-most column of Table~\ref{tab:few_shot_learning}, titled Few-Shot.  These results show that the detector can very accurately transfer to detect new generators through few-shot learning.  In each case, the detector achieves an AUC of 0.98 or higher.  This is a substantial increase over the AUCs achieved through zero-shot transferability.  

Notably, for Sora we increase the AUC from 0.530 to 0.982 through few-shot learning.  This corresponds to an AUC boost of 0.452 and an RER of 96\%. %96.1
%
These results show that synthetic video detectors can be transfered to reliably detect new generators through few-shot learning.  This is particularly important given the rapid pace with which new generators such as Sora are continually emerging.


%we fine-tuned our detector that was pre-trained using data form all four generators in the training set. As before, we 


\begin{comment}

\hrulefill

In this section, we investigate how few-shot learning can be used to adapt an existing pretrained detector to detect emerging video generation sources. To do this, we first took MISLnet~\cite{bayar2016deep,openset}, the best performing architecture in prior experiments in our paper, and trained this network architecture on the entire set of real and synthetic training videos in our dataset (described in Sec.~\ref{subsec:common_exp_setup}). Then, we tested this network on three new and emerging video generation sources: Sora~\cite{sora}, Pika~\cite{Pika}, and VideoCrafter v2~\cite{videocrafter2} to get a zero-shot transference baseline. And finally, we applied few-shot learning over this system and evaluate its few-shot performance over each sources.
Specifically, we performed few-shot learning by fine-tuning the pre-trained detector using only 50 seconds of video from each generation sources and tested on 5,000 video frames from Sora\cite{sora}, 10,000 video frames from Pika\cite{Pika}, and 10,000 video frames from VideoCrafter v2\cite{videocrafter2}.
We reported the results of this experiment in Tab.~\ref{tab:few_shot_learning}.

Tab.~\ref{tab:few_shot_learning}'s results show that MISLnet\cite{bayar2016deep,openset} achieved low amount of zero-shot transference on Sora~\cite{sora}, some level of zero-shot transference on Pika~\cite{Pika}, and high level of transference on VideoCrafter v2~\cite{videocrafter2}. However, when this network is allowed to see only 50 seconds of video from each generation source, MISLnet\cite{bayar2016deep,openset} displayed strong detection performance across all sources. This suggests that few-shot learning can be leveraged to address the challenge of detecting novel synthetic videos made using new generation techniques. 
\end{comment}

==> sec/LearningSynthVid_v4.tex <==


\section{Learning Synthetic Video Forensic Traces}
\label{sec:learn_synth_vid_traces}

Results presented in the previous two sections show that the traces left by synthetic video generators are different than those left by image generators, and that synthetic image detectors do not reliably detect these traces.

In this section, however, we show that synthetic video traces can be learned.  Through a series of experiments, we show that CNNs can be trained to accurately perform synthetic video detection and generator source attribution.   
Furthermore, we demonstrate that robust training can make these detectors perform strongly even in the presence of H.264 re-compression.  Additionally, we show how video-level detection can be performed to boost performance over frame-level detection.

\input{sec/ExSetupVid_v5_DSV}

\input{sec/Exp1_SynthVidDet_v4}

\input{sec/Exp2_SynthVidAttr_v5_DSV}

\input{sec/Exp3_Recompression_v4}

\input{sec/Exp4_VideoLevelDet_v4}












==> sec/SynthVidTraces_v1.tex <==
% SynthVidTraces_v1

\section{Synthetic Video Traces}
\label{sec:synth_video_traces}

Considering the findings of previous section, it would be reasonable to assume that synthetic video generators have significantly different forensic traces compared to synthetic image generators where even after eliminating the effects of video compression synthetic image detectors are not able to have sufficient performance when it comes to detecting synthetic videos.

In order to have a qualitative demonstration of this claim we decided to visualize low-level synthetic image generator and video generator traces and compare them together. We do this using the same method used in \citethis where we use the de-noising network from \citethis to de-noise the synthetic image or frames of the synthetic video subtract them from the original and visualize the spectral analysis as demonstrated in \citethis. 


Figure 1, allows us to have a better understanding of the traces left behind by each generator, being synthetic image or video generator, we can see that the visualization of the traces from  ProGAN\citethis,  and StyleGAN3\citethis, StarGANM\citethis, CycleGAN\citethis have a significantly different shape from the visualization for Cogvideo\citethis and  Luma\citethis, sora \citethis, pika\citethis. However, the trace visualization from VideoCrafter \citethis is closely similar to the one from latent diffusion\citethis and interestingly although the trace visualization from Stable Image Diffusion v 1.9 \citethis is close to the trace visualization for Stable Video Diffusion\citethis created using the same images from Stable Image Diffusion v1.9 \citethis, in some areas they are distinguishable from each other for instance the traces from stable image diffusion are more densely populated around the x axis which would explain the drop in performance observed in synthetic image detectors.

To delve deeper in this analysis, we observer regularly appearing dots in the synthetic image generators which can be attributed to the up-sampling operation traces commonly used in U-net style networks as demonstrated by \citethis. However, most synthetic video generators largely lack this structure.

We know that synthetic video generators employ significantly different architectures compared to synthetic image generators and for that reason the pattern observer in their trace visualization is drastically different from one another. Moreover we see that different families of generators, depending if they use Diffusion models, Transformers, Neural Radiance Fields or a combination of those have significantly different traces we can see this point illustrated by comparing the visualizations from Sora \citethis and Luma \citethis that are ,respectively, Neural Radiance Field and combination based we can see that the visualization is significantly different from any other generator. 

==> sec/SynthVidTraces_v2_MCS.tex <==
% SynthVidTraces_v1_MCS

\section{Synthetic Video Forensic Traces}
\label{sec:synth_video_traces}

Here, we present evidence that forensic traces in synthetic video are substantially different than forensic traces in synthetic images.  We qualitatively demonstrate this by visualizing the low-level forensic traces left by a number of different image and video generators using the approach proposed in~\cite{resnet34_method}. %by Zhang et al.~\citethis.



To do this, we collected a set of 1000 images and video frames created using several different image and video generators.  These image generators included ProGAN~\cite{progan}, CycleGAN~\cite{cyclegan}, StarGAN~\cite{stargan}, StyleGAN 3~\cite{stylegan3}, Latent Diffusion~\cite{diffusion7}, and Stable Diffusion~\cite{stablediffusion}, while video generators included Luma~\cite{Luma}, VideoCrafter v1~\cite{videocrafter1}, CogVideo~\cite{cogvideo}, Pika~\cite{Pika}, Sora~\cite{sora}, and Stable Video Diffusion~\cite{stablevideo}. 
%
We then created a noise residual for each image and video frame $x_k$ by denoising it using a denoising algorithm $\phi$, then subtracting the denoised image or frame from the original.  
All noise residuals from a single generator were averaged to produce an aggregate noise residual $y= \tfrac{1}{N}\sum_{k=1}^{N}x_k-\phi(x_k)$.  Frequency domain representations of these aggregate noise residuals were then created by taking their Fourier transforms, then their magnitudes were ploted to produce trace visualizations.

The resulting low-level forensic traces for each image and video generator are shown in Fig.~\ref{fig:trace_visualization}.  By examining these traces, we can clearly see that synthetic images contain substantially different traces than synthetic videos.    This is especially true for video generators such as Luma and Pika, which exhibit a strong cloud-like pattern around the origin.

The significant difference between forensic traces left by 
%video generators as opposed to image generators 
image and video generators 
is likely the major reason that synthetic image detectors exhibit substantially lower performance on video.  Even when robustly trained, synthetic image detectors learn features to capture forensic traces similar to what they have seen before.  Since video traces can be substantially different in nature, the features learned synthetic image detectors are not well suited to capture these traces.  

We note that this aligns with findings of prior research.  For example, Corvi et al.~\cite{luisa} found that Stable and Latent diffusion models produce different forensic traces than image generators such as ADM and DALL-E 2.  Furthermore, they found that even robustly trained synthetic image detectors ``still cannot reliably detect images that present artifacts significantly different from those seen during training.''~\cite{luisa}

\subheader{Differences Between Image and Video Generation}
%The reason that video generators exhibit significantly different traces than image generators is that 
A major reason that video generators exhibit significantly different traces than image generators is because they typically utilize very different generation approaches and architectures.  For example, traces left by image generators typically include periodic spectral peaks or a grid-like structure that Zhang et al.~\cite{zhang2019detecting} showed are caused by upsampling operations used in a generator's architecture.  By contrast, some video generation techniques such as Luma employ neural radiance fields (NeRFs) or other architectures that do not utilize upsampling.  As a result, the distinct periodic peak or grid-like patterns typically found in synthetic image traces will not be present in traces from these video generators.
%Other generators utilize emerging architectures or approaches.  

Additionally, other generators produced by industry may utilize emerging architectures or approaches that are undisclosed or only partially disclosed to protect trade secrets.  For example, full details about Pika's generation are not currently publicly available.  However, the significant difference between its traces and those of other generators suggest that Pika uses a noticeably different generation technique.

==> sec/SynthVidTraces_v3_Tai.tex <==
% SynthVidTraces_v1_MCS



\section{Synthetic Video Forensic Traces}
\label{sec:synth_video_traces}



Here, we present evidence that forensic traces in synthetic video are substantially different than forensic traces in synthetic images.  We qualitatively demonstrate this by visualizing the low-level forensic traces left by a number of different image and video generators using the approach proposed in~\cite{resnet34_method}. %by Zhang \etal~\citethis.

To do this, we collected a set of 1000 images and video frames created using several different image and video generators.  These image generators included ProGAN~\cite{progan}, CycleGAN~\cite{cyclegan}, StarGAN~\cite{stargan}, StyleGAN 3~\cite{stylegan3}, Latent Diffusion~\cite{diffusion7}, and Stable Diffusion~\cite{stablediffusion}, while video generators included Luma~\cite{Luma}, VideoCrafter v1~\cite{videocrafter1}, CogVideo~\cite{cogvideo}, Pika~\cite{Pika}, Sora~\cite{sora}, and Stable Video Diffusion~\cite{stablevideo}. 
%
We then created a noise residual for each image and video frame $x_k$ by denoising it using a denoising algorithm $\phi$, then subtracting the denoised image or frame from the original.  
All noise residuals from a single generator were averaged to produce an aggregate noise residual $y= \tfrac{1}{N}\sum_{k=1}^{N}x_k-\phi(x_k)$.  Frequency domain representations of these aggregate noise residuals were then created by taking their Fourier transforms, then their magnitudes were ploted to produce trace visualizations.



\subheader{Image and Video Generator's Trace Comparison}
The resulting low-level forensic traces for each image and video generator are shown in Fig.~\ref{fig:trace_visualization}.  By examining these traces, we can clearly see that synthetic images contain substantially different traces than synthetic videos.
For example, traces left by image generators (e.g. ProGAN, CycleGAN, Latent Diffusion) typically include periodic spectral peaks or a grid-like structure that Zhang \etal~\cite{zhang2019detecting} showed are caused by upsampling operations used in a generator's architecture.  By contrast, some video generation techniques such as Luma employ neural radiance fields (NeRFs) or other architectures that do not utilize upsampling.  As a result, the distinct patterns often seen in synthetic image traces will not be present in traces from these video generators.

Additionally, other generators produced by industry may utilize emerging techniques that are undisclosed to protect trade secrets. For example, while the full details about Pika's generation are not currently publicly available, the significant difference between its traces and others' traces suggest that Pika uses a noticeably different generation technique.

Due to the stark differences between forensic traces left by image and video generators, it is highly likely that this is the major reason why synthetic image detectors exhibit substantially lower performance on video.  Even when robustly trained, synthetic image detectors learn features to capture forensic traces similar to what they have seen before.  Since video traces can be substantially different in nature, the features learned synthetic image detectors are not well suited to capture these traces.  

We note that our findings align with prior research. Specifically, Corvi \etal~\cite{luisa} found that Stable and Latent diffusion models produce different forensic traces than image generators such as ADM and DALL-E 2.  They also showed that even robustly trained synthetic image detectors ``still cannot reliably detect images that present artifacts significantly different from those seen during training.''~\cite{luisa}

==> sec/Transferability_v1.tex <==
% Transferability_v1

\section{Zero-shot and Few Shot Transferability of Synthetic Video Detectors}
\label{sec:zero_few_shot_transfer}


\subsection{Detection Transferability}
With the rapid development of new synthetic video generation methods and emergence of novel video generation methods transferability is of high value for any detection system. To evaluate the transferability of the detector we run an experiment where we  train the network on three of the generators from our training data set and test it on the remaining one. In addition to that, we run an experiment where we train the network on all four generators but test it on a new generator that it has not seen before.

\subheader{Experimental Setup}
For our training datasets we use 40,000 frames from each of the CogVideo\citethis, Luma\citethis, VideoCrafter\citethis and Stable Video Diffusion\citethis. Morevoer, for testing we use 10,0000 frames from each of those datasets and for the real videos we use equivalent number of frames to have a balanced dataset from the Moments in Time\citethis and VideoASID\citethis datasets. Moreover, we use the MISLnet\citethis network for this experiment.

\subheader{Transferability Evaluation}
As seen in Table 5, when the detector has not seen any examples from the test generator the performance is significantly deprecated.

However, if at list one generator from the same family is present in the training data the performance drop is significantly less than when there is no generator from the same family present in the training data. For instance, VideoCrafter\citethis and Stable Video Diffusion \citethis both use a diffusion model in their generator. Hence, when we train the detector on a set of data that includes one of them the AUc is significantly higher than when the detector is not trained on any data from the same family of generators such is the case for training the detector on diffusion and transformer based generators and testing it on Luma\citethis which is a Neural Radiance Field based Generator.

This point is further solidified when we see the results of training on a dataset that includes videoCrafter v1\citethis but tested on a dataset from videos generated by VideoCrafter v2\citethis. In this case, we observe that the presence of data that is largely similar in training data improves the transferability significantly.

In addition, when we train the detector on data that is not in the same family of generators as the test generator the performance of the detector is close to random much lower. For instance, Sora \citethis uses a completely different generator from the other generators mentioned in this paper and as a result when we train the detector on data from Luma\citethis,Stable Video Diffusion\citethis, CogVideo\citethis and VideoCrafter\citethis and test it on Sora\citethis the detector performance is close to random guess.

\subsection{Few Shot Learning}
A method to make the detector transfer better to new generators is to fine-tune the pre-trained detectors using a few samples from the new generator. This procedure is known as few shot learning and allows us to increase the performance of the detector on novel synthetic video generators to a sufficient level.

\subheader{Experimental Setup}
For this experiment, we train MISLnet\citethis using 40,000 frames from  videos generated by Luma\citethis, CogVideo\citethis, VideoCrafter v1\citethis and Stable Video Diffusion \citethis each and 80,000 frames from real videos  in Moments in Time\citethis and VideoASID\citethis each. Afterwards, we fine-tune the resulting detector using 50 seconds of video from each of the new generators including SORA\citethis, Pika\citethis and VideoCrafter v2 \citethis.

\subheader{Few Shot Learning Evaluation}
As we can see in table 6 the process of few shot learning improves the performance of the detector significantly. For instance with zero-shot learning the detector was close to random guess when it came to detecting SORA\citethis. However, with few-shot learning the detector is able to detect SORA\citethis videos with an AUC of 0.996.

In contrast, the performance of the detector on VideoCrafter v2 \citethis improves minimally after few-shot learning. However, this could be attributed to the fact that the detector has had the chance to see the traces from VideoCrafter v1 \citethis in the training process and already is able to detect videocrafter v2\citethis without seeing them with an AUC of 0.939.

In conclusion, few-shot learning allows us to make the detector adaptable to any new generators that emerge. With minimal training and limited data we are able to adapt a detector to to perform sufficiently on any novel synthetic video generator

==> sec/Transferability_v2_Tai.tex <==
% Transferability_v1

\section{Zero-shot and Few Shot Transferability of Synthetic Video Detectors}
\label{sec:zero_few_shot_transfer}

Novel synthetic video generation architectures and methods are rapidly emerging. Hence, in this section, we further evaluate the ability of trained synthetic video detectors to detect synthetic videos from new and unseen generation sources. To comprehensively understand the challenges of this problem, we performed two experiments: Experiment 1 shows how these detectors adapt to completely new synthetic video sources in a leave-one-out training and testing methodology; and Experiment 2 shows how these detectors can leverage few-shot learning to better detect popular emerging video generation sources such as Sora~\citethis, Pika~\citethis, and VideoCrafter v2~\citethis.

\subsection{Experiment 1: Zero-shot Transferability}
\label{subsec:exp_zero_shot}

In this experiment, we explore the ability of synthetic video detectors to detect synthetic videos from new and unseen generation sources. To accomplish this, we used our synthetic video dataset (detailed in Sec.~\ref{subsec:common_exp_setup}) to train and evaluate our detectors on different video generation sources in a leave-one-out manner. For examples, out of the four video generation sources in our dataset (Luma, CogVideo, VideoCrafter-v1, and Stable Video Diffusion), we would pick one source to be the unseen source (e.g. Luma) and train our model on the other three sources (e.g. CogVideo, VideoCrafter-v1, Stable Video Diffusion). We repeated this experiment for all possible combination of seen and unseen sources, and reported the result of each experiment in Tab.~\ref{tab:exp_leave_one_out}. 

Results presented in Tab.~\ref{tab:exp_leave_one_out} show that the best performing architecture in prior experiments in this paper, MISLnet~\citethis, achieves high performance on the testing video of the seen generation sources but obtained a significant drop in performance when tested on the unseen, left-out source. This is not surprising, however, because the forensic traces from the unseen source are distinct from those seen during training. In the next section, we will explore how we can utilize few-shot learning to address this challenge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experiment 2: Few-shot Learning for Emerging Generation Sources}
\label{subsec:exp_few_shot}

In this section, we investigate how few-shot learning can be used to adapt an existing pretrained detector to detect emerging video generation sources. To do this, we first took MISLnet~\citethis, the best performing architecture in prior experiments in our paper, and trained this network architecture on the entire set of real and synthetic training videos in our dataset (described in Sec.~\ref{subsec:common_exp_setup}). Then, we tested this network on three new and emerging video generation sources: Sora~\citethis, Pika~\citethis, and VideoCrafter v2~\citethis to get a zero-shot transference baseline. And finally, we applied few-shot learning over this system and evaluate its few-shot performance over each sources.
Specifically, we performed few-shot learning by fine-tuning the pretrained detector using only 50 seconds of video from each generation sources and tested on \TODO{X number} of video frames from Sora, \TODO{X number} of video frames from Pika, and \TODO{X number} of video frame from VideoCrafter v2.
We reported the results of this experiment in Tab.~\ref{tab:few_shot_learning}.

Tab.~\ref{tab:few_shot_learning}'s results show that MISLnet achieved low amount of zero-shot transference on Sora~\citethis, some level of zero-shot transference on Pika~\citethis, and high level of transference on VideoCrafter v2~\citethis. However, when this network is allowed to see only 50 seconds of video from each generation source, MISLnet displayed strong detection performance across all sources. This suggests that few-shot learning can be leveraged to address the challenge of detecting novel synthetic videos made using new generation techniques. 


==> sec/Video_Compression_Effects.tex <==
\subsection{Video Compression Effects}
Videos can go through the process of re-compression for a multitude of reasons, when we upload a video to internet video sharing websites, in most cases,the video is recompressed with multiple re-compression factos. As demonstrated in \citethis, we know that compression artifacts can have a significant effect on the performance of detectors. When a video goes through the process of re-compression depending on the re-compression factor we may a range of difference in detector performance ranging from little to no difference to sizable performance drops in detector performance. \\
\indent To evaluate the robustness of our detector when it comes to re-compression we take the videos used to train the detector and recompress them with a range of compression factors. 
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment was trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time\citethis and VideoASID\citethis and for synthetic videos we used videos from CogVideo\citethis,VideoCrafter\citethis, Stable Video Diffusion\citethis and Luma \citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment. All of the frames were also separately recompressed with factors ranging from CRF-0 to CRF-40\\
\textbf{Compression Effects Evaluation.}
As showcased in the table, different compression factors have different effects on the performance of the network. To summarize for lower compression factors such as CRF-0 and CRf-10 the effect on detector performance is minimal ranging from 0.01-0.04 drop in AUC.\\
\indent For CRF-20 we can almost see no effect on performance when we test the network trained on regular videos on videos recompressed with this compression factor which is to be expected since the default compression factor for videos is CRF-23 and CRF-20 is very close to that so the network is already familiar with the artifacts from this compression factor.\\
\indent In contrast, when we use CRF-30 and CRF-40 the effect on detector performance is significantly larger where when tested on videos recompressed with CRF-30 the network is on average has a 0.13 worse AUC across all generators and this number only rises when using CRF-40 as the compression factor, reaching 0.29 drop in AUC.\\
\include{tables/recompression1}
\indent We can conclude that re-compression can make the task of detecting synthetically generated videos more challenging and the higher the re-compression factor is the harder it is to accurately detect the synthetic video.
\indent To be able to accurately detect videos even after re-compression, one solution is to robust train our network against re-compression. In this process, we train the same detector with the same data with the only difference being the video frames have now been re-compressed with a multitude of compression factors.\\
\textbf{Robust Trainng Results.} As shown in table after testing the robust trained network the variation in performance going from non re-compressed frames to re-compressed frame shrinks significantly. For CRF-0 and CRF-10 the drop in AUC lowers from an average of 0.03 to 0.01, and for CRF-30 and CRF-40 where, respectively, we were seeing 0.13 and 0.29 drops in AUC now that number has changed to only 0.01 and 0.03 average drop in AUC across all generators.\\
\indent Based on the results of this experiment we can conclude that we can make our detectors invulnerable to re-compression artifacts by robust training them using a multitude of compression artifacts.

==> sec/ZeroShotTransfer_v3_DSV.tex <==
% Transferability_v1

\input{tables/ood_dataset_stats}

\section{Zero-shot and Few Shot Transferability of Synthetic Video Detectors}
\label{sec:zero_few_shot_transfer}

\input{tables/table_one_out}

Novel synthetic video generation architectures and methods are rapidly emerging. Hence, in this section, we further evaluate the ability of trained synthetic video detectors to detect synthetic videos from new and unseen generation sources. To comprehensively understand the challenges of this problem, we performed two experiments: Experiment 1 shows how these detectors adapt to completely new synthetic video sources in a leave-one-out training and testing methodology; and Experiment 2 shows how these detectors can leverage few-shot learning to better detect popular emerging video generation sources such as Sora~\cite{sora}, Pika~\cite{Pika}, and VideoCrafter v2~\cite{videocrafter2}.

\subsection{Experiment 1: Zero-shot Transferability}
\label{subsec:exp_zero_shot}

In this experiment, we explore the ability of synthetic video detectors to detect synthetic videos from new and unseen generation sources. To accomplish this, we used our synthetic video dataset (detailed in Sec.~\ref{subsec:common_exp_setup}) to train and evaluate our detectors on different video generation sources in a leave-one-out manner. For examples, out of the four video generation sources in our dataset (Luma, CogVideo, VideoCrafter-v1, and Stable Video Diffusion), we would pick one source to be the unseen source (e.g. Luma) and train our model on the other three sources (e.g. CogVideo, VideoCrafter-v1, Stable Video Diffusion). We repeated this experiment for all possible combination of seen and unseen sources, and reported the result of each experiment in Tab.~\ref{tab:exp_leave_one_out}. 

Results presented in Tab.~\ref{tab:exp_leave_one_out} show that the best performing architecture in prior experiments in this paper, MISLnet~\cite{bayar2016deep,openset}, achieves high performance on the testing video of the seen generation sources but obtained a significant drop in performance when tested on the unseen, left-out source. This is not surprising, however, because the forensic traces from the unseen source are distinct from those seen during training. In the next section, we will explore how we can utilize few-shot learning to address this challenge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sec/ZeroShotTransfer_v4_MCS.tex <==

\input{tables/ood_dataset_stats}

%\section{Zero-shot and Few Shot Transferability of Synthetic Video Detectors}
%\section{Detection Transferability to New Video Generators}
\section{Detection Transferability to New Generators}

Currently, new synthetic video generator architectures and generation approaches are emerging at a rapid pace.  Because of this, it is important to understand the transferability of synthetic image detectors to new generators.  
%
In this section, we conduct a series of experiments to examine synthetic video detectors transferability in both zero-shot and few-shot transfer scenarios. 

%We show that while it can be difficult to detect synthetic videos generated using approaches that are substantially different than seen during training


\label{sec:zero_few_shot_transfer}

\input{tables/table_one_out}

%Novel synthetic video generation architectures and methods are rapidly emerging. Hence, in this section, we further evaluate the ability of trained synthetic video detectors to detect synthetic videos from new and unseen generation sources. To comprehensively understand the challenges of this problem, we performed two experiments: Experiment 1 shows how these detectors adapt to completely new synthetic video sources in a leave-one-out training and testing methodology; and Experiment 2 shows how these detectors can leverage few-shot learning to better detect popular emerging video generation sources such as Sora~\cite{sora}, Pika~\cite{Pika}, and VideoCrafter v2~\cite{videocrafter2}.

%\subsection{Experiment 1: Zero-shot Transferability}
\subsection{Zero-Shot Transferability}
\label{subsec:exp_zero_shot}

In our first set of experiment, we examined synthetic video detectors' zero-shot transferability performance.  This corresponds to a detector's ability to detect videos from a new generator without any retraining. 

We began by training the best performing detector (MISLnet) using data from three of the generators in our training set. We benchmarked the detector's performance on the portion of the test dataset corresponding to these generators seen during training.  After this, we measured the detector's zero-shot transferability performance by using to detect videos `unseen'' generator using its corresponding testing data.  

Results from this experiment are presented are in Table~\ref{tab:exp_leave_one_out}.  
%As we saw in the results presented in Section~\
These results show that while the detector achieves strong performance on videos from generators seen during training, performance drops significantly when evaluating on new generators.  Specifically, the AUC drops from an average of 0.990 for ``seen'' generators to an average of 0.727 for new, ``unseen'' generators.  

We conducted a similar experiment, in which we used the detector trained on all four generators in our training set to detect synthetic videos from the generators in our Out-of-Distribution testing set described in Section~\ref{subsec:common_video_exp_setup}. These videos were generated using three different generators: Sora, Pika, and VideoCrafter v2.

The results of this experiment are presented in the second colum of Table~\ref{tab:few_shot_learning}, labeled ``Zero-Shot''.  These experiments yielded similar results, in which the detector had significant difficulty detecting videos from these new, unseen generators. 
%
The only notable exception to this was VideoCrafter v2, whose generator architecture strongly resembles VideoCrafter v1.


The results of these experiments are somewhat unsurprising.  As we can see from the generator trace visualizations in Fig.~\ref{fig:trace_visualization}, traces left by different generators can vary substantially.  Furthermore, we know that both video generator architectures and generation approaches (i.e. NeRF, diffusion model, transformer, etc.) vary significantly from generator to generator.  As a result, it is  difficult for a detector to capture traces from new generation that leave different traces than those seen in training. 
We also note, this aligns with similar findings obtained for synthetic image detection~\cite{luisa}. %corvi




% In this experiment, we explore the ability of synthetic video detectors to detect synthetic videos from new and unseen generation sources. To accomplish this, we used our synthetic video dataset (detailed in Sec.~\ref{subsec:common_exp_setup}) to train and evaluate our detectors on different video generation sources in a leave-one-out manner. For examples, out of the four video generation sources in our dataset (Luma, CogVideo, VideoCrafter-v1, and Stable Video Diffusion), we would pick one source to be the unseen source (e.g. Luma) and train our model on the other three sources (e.g. CogVideo, VideoCrafter-v1, Stable Video Diffusion). We repeated this experiment for all possible combination of seen and unseen sources, and reported the result of each experiment in Tab.~\ref{tab:exp_leave_one_out}. 

%Results presented in Tab.~\ref{tab:exp_leave_one_out} show that the best performing architecture in prior experiments in this paper, MISLnet~\cite{bayar2016deep,openset}, achieves high performance on the testing video of the seen generation sources but obtained a significant drop in performance when tested on the unseen, left-out source. This is not surprising, however, because the forensic traces from the unseen source are distinct from those seen during training. In the next section, we will explore how we can utilize few-shot learning to address this challenge.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




==> sec/intro_v1.tex <==
% intro_v1

\section{Introduction}

%Rough sketch of intro below

Over the last several years, significant advances in generative AI have led to development of multiple new approaches to create visually realistic synthetic images.  At the same time, approaches such as  CLIP\cite{clip} have been developed, when enable latent space image representations to be guided by text prompts.  As a result, a number of text-prompted synthetic image generation systems have been created by both researchers and industry, and are widely available to the general public.

The ability to create visually convincing synthetic images has caused a major misinformation and disinformation threat.  Synthetic images can easily be created by anyone, then used as visual evidence of a fake event in order to mislead a target audience.

To combat this, researchers have developed a number of techniques to detect synthetic images.  These techniques operate by searching for statistical traces present inside synthetic images that are left by their source generator.  For example, prior work by Zhang et al. has shown that the upsampling operation used in many generator architectures to grow an image from a small latent representation to a full sized image leaves behind traces similar to those left by resampling~\cite{resnet34_method}.  A number of approaches have been successfully developed to accurately detect synthetic images made by a wide variety of generators~\cite{luisa,genimage,swin_method2,resnet_method_2,resnet34_method2,resnet34_method3,resnet50_method4,vgg16_method3,xception_method3} and attribute them to their source~\cite{dif,genimage,openset}

% we should be sure to cite our open set attributino stuff

Very recently, AI-based synthetic video generators have begun to emerge.  These range from text-prompted approaches such as Stable Video Diffusion, VideoCrafter, or OpenAI's recently released Sora, %to others which enable the creation and manipulation of synthetic videos based on a set of image
to others such as Luma AI's NeRF-basesd approach which allows synthetic videos to be generated and manipulated based on a set of input images.  
The emergence of synthetic video generators represents not only a major technological advancement, but also a significant escalation in the potential misinformation and disinformation threats caused by generative AI.

One would reasonably assume that synthetic image detectors should accurately detect synthetic videos.  In this paper, however, we demonstrate that synthetic image detectors do not accurately detect synthetic videos.  Furthermore, we demonstrate that this is not caused due to factors detector performance degradation due to H.264 compression.  Instead, we show that synthetic video generators leave behind traces that are significantly different than those left by synthetic image generators, and which synthetic image detectors are not trained to detect.  Encouragingly, we show that synthetic video traces can be accurately learned and utilized to perform accurate synthetic video detection and generator source attribution.  Furthermore, we examine the transferability of synthetic video detectors to identify videos generated by generators not encountered during training.  Our results show that using only a small amount of video from new generators, pretrained synthetic video detectors can be transferred to accurately detect new generators.





The novel contributions of this paper are listed below:
\begin{itemize}
    \item We show that synthetic image detectors do not reliably detect AI-generated synthetic videos.  This holds true even after robust training against H.264 compression.

    \item We demonstrate that synthetic video generators leave behind substantially different traces than synthetic image generators.  This is the primary cause of synthetic image detectors' poor performance on video.

    \item We show that synthetic video traces can be learned and used to perform reliable synthetic video detection and generator source attribution.  Furthermore, we show that theses detectors can be robustly trained to overcome negative effects caused by H.264 compression.

    \item We demonstrate that zero-shot transferability, i.e. when synthetic video detectors are used to detect videos from new generators, is challenging.  However, we also show how few-shot transferability can be achieved so that synthetic videos new video generators can be accurately detected using a comparatively small amount of fine tuning data.

    \item We create a new dataset of synthetic videos from a number of different generators that can be used to train and benchmark the performance of synthetic video detectors.  
    
\end{itemize}


==> sec/intro_v2_DSV.tex <==
% intro_v1

\section{Introduction}

%Rough sketch of intro below

Over the last several years, significant advances in generative AI have led to development of multiple new approaches to create visually realistic synthetic images.  At the same time, approaches such as  CLIP\cite{clip} have been developed, when enable latent space image representations to be guided by text prompts.  As a result, a number of text-prompted synthetic image generation systems have been created by both researchers and industry, and are widely available to the general public.

The ability to create visually convincing synthetic images has caused a major misinformation and disinformation threat.  Synthetic images can easily be created by anyone, then used as visual evidence of a fake event in order to mislead a target audience.

To combat this, researchers have developed a number of techniques to detect synthetic images.  These techniques operate by searching for statistical traces present inside synthetic images that are left by their source generator.  For example, prior work by Zhang et al. has shown that the upsampling operation used in many generator architectures to grow an image from a small latent representation to a full sized image leaves behind traces similar to those left by resampling~\cite{resnet34_method}.  A number of approaches have been successfully developed to accurately detect synthetic images made by a wide variety of generators~\cite{luisa,genimage,swin_method2,resnet_method_2,resnet34_method2,resnet34_method3,resnet50_method4,vgg16_method3,xception_method3} and attribute them to their source~\cite{dif,genimage,openset}

% we should be sure to cite our open set attributino stuff

Very recently, AI-based synthetic video generators have begun to emerge.  These range from text-prompted approaches such as Stable Video Diffusion, VideoCrafter, or OpenAI's recently released Sora, %to others which enable the creation and manipulation of synthetic videos based on a set of image
to others such as Luma AI's NeRF-basesd approach which allows synthetic videos to be generated and manipulated based on a set of input images.  
The emergence of synthetic video generators represents not only a major technological advancement, but also a significant escalation in the potential misinformation and disinformation threats caused by generative AI.


One might expect synthetic image detectors to effectively identify synthetic videos. However, our research reveals that synthetic image detectors struggle with this task. Importantly, this is not due to performance degradation caused by H.264 compression. Instead, synthetic video generators leave distinct traces undetected by image detectors. Fortunately, we demonstrate that these unique traces can be learned for accurate detection and source attribution. Additionally, we investigate the transferability of synthetic video detectors to new generators and unseen data, finding promising results with minimal training data.





The novel contributions of this paper are listed below:
\begin{itemize}
    \item We show that synthetic image detectors do not reliably detect AI-generated synthetic videos.  This holds true even after robust training against H.264 compression.

    \item We demonstrate that synthetic video generators leave behind substantially different traces than synthetic image generators.  This is the primary cause of synthetic image detectors' poor performance on video.

    \item We show that synthetic video traces can be learned and used to perform reliable synthetic video detection and generator source attribution.  Furthermore, we show that theses detectors can be robustly trained to overcome negative effects caused by H.264 compression.

    \item We demonstrate that zero-shot transferability, i.e. when synthetic video detectors are used to detect videos from new generators, is challenging.  However, we also show how few-shot transferability can be achieved so that synthetic videos new video generators can be accurately detected using a comparatively small amount of fine tuning data.

    \item We create a new dataset of synthetic videos from a number of different generators that can be used to train and benchmark the performance of synthetic video detectors.  
    
\end{itemize}


==> sec/old_or_temp/0_abstract.tex <==
\begin{abstract}
The ABSTRACT is to be in fully justified italicized text, at the top of the left-hand column, below the author and affiliation information.
Use the word ``Abstract'' as the title, in 12-point Times, boldface type, centered relative to the column, initially capitalized.
The abstract is to be in 10-point, single-spaced type.
Leave two blank lines after the Abstract, then begin the main text.
Look at previous \confName abstracts to get a feel for style and length.
\end{abstract}

==> sec/old_or_temp/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/old_or_temp/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/old_or_temp/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.

==> sec/old_or_temp/Det_Attrib_v1.tex <==
% Det_Attrib_v1

\section{Learning Synthetic Video Traces for Detection and Source Attribution}

Knowing that different generators leave different traces behind we conduct experiments to learn each and all of these traces to be able to accurately detect synthetically generated videos.

\subsection{Synthetic Image Detection}

In synthetic image generators the network has significant upsampling traces left behind due to starting from an image and repeatedly up-sampled until the desired outcome has been achieved this is know to be especially the case for Generative Adversarial Networks~\citethis. However, due to the drop in the performance of synthetic image detectors and the observation in the previous section it would be reasonable to assume that this is not the case for synthetic video generators.

As a result, we use a multitude of forensic architectures to try and learn the traces left behind by the synthetic video generators where instead of training the detector on synthetic images we train the network using frames extracted from videos generated by different synthetic video generation methods.

\subheader{Metrics} AUC

\subheader{Training Data} The networks used in this experiment were trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time~\citethis and VideoASID~\citethis and for synthetic videos we used videos from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment.

\subheader{Video Benchmarking data} The performance of the synthetic video detector network in detecting synthetic videos accurately was benchmarked using 10,000 synthetic frames from each synthetic video generator from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis and 20,000 real video frames from a subset of datasets Moments in Time~\citethis and VideoASID~\citethis.

\subheader{Video-based Detector Evaluation} As demonstrated in Table3, the same detectors used for detecting synthetic image when trained on synthetic video data can achieve the sufficient AUCs for accurate detection we can see the average AUC rising to 0.956 whereas when we used the same detectors trained on synthetic images the average AUC was only 0.704 even after robust training on recompressed data. In Addition, we observe that the best detector to be used for this cas is Mislnet~\citethis with the testing AUC of 0.982 outperforming the other detectors by at least 0.012 under equal conditions.

From this experriment we can deduce that although synthetically generated videos are not hard to detect the detectors still need to be trained on suitable data to learn the novel traces left behind by the synthetic video generators in order to be able to detect them with sufficient performance.


\subsection{Generator Source Attribution}

While detection is the most important issue when it comes to synthetic videos, source attribution is of equal importance. Moreover, since the traces from different generators vary from one another significantly we can easily use a multi-class classifier to tackle the problem of source attribution.
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment were trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time~\citethis and VideoASID~\citethis and for synthetic videos we used videos from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment.\\
\textbf{Video Benchmarking data.} The performance of the synthetic video attribution network in detecting synthetic images accurately was benchmarked using 10,000 synthetic frames from each synthetic video generator from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis and 20,000 real video frames from a subset of datasets Moments in Time~\citethis and VideoASID~\citethis.\\
\textbf{Video Source Attribution Evaluation} As we can see in Table 5. using the same base architecture we used for detection and the same data and changing the task from binary classification, detection, to multi-class classification we are able to attribute each video to its source generator with a testing AUC of 0.985. This finding further solidifies the idea that synthetic video traces are not only distinct from synthetic image traces but are also significantly distinguishable from each other.

\subsection{Effects of Video Compression}

Videos can go through the process of re-compression for a multitude of reasons, when we upload a video to internet video sharing websites, in most cases,the video is recompressed with multiple re-compression factos. As demonstrated in ~\citethis, we know that compression artifacts can have a significant effect on the performance of detectors. When a video goes through the process of re-compression depending on the re-compression factor we may a range of difference in detector performance ranging from little to no difference to sizable performance drops in detector performance. \\
\indent To evaluate the robustness of our detector when it comes to re-compression we take the videos used to train the detector and recompress them with a range of compression factors.
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment was trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time~\citethis and VideoASID~\citethis and for synthetic videos we used videos from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment. All of the frames were also separately recompressed with factors ranging from CRF-0 to CRF-40\\
\textbf{Compression Effects Evaluation.}
As showcased in the table, different compression factors have different effects on the performance of the network. To summarize for lower compression factors such as CRF-0 and CRf-10 the effect on detector performance is minimal ranging from 0.01-0.04 drop in AUC.\\
\indent For CRF-20 we can almost see no effect on performance when we test the network trained on regular videos on videos recompressed with this compression factor which is to be expected since the default compression factor for videos is CRF-23 and CRF-20 is very close to that so the network is already familiar with the artifacts from this compression factor.\\
\indent In contrast, when we use CRF-30 and CRF-40 the effect on detector performance is significantly larger where when tested on videos recompressed with CRF-30 the network is on average has a 0.13 worse AUC across all generators and this number only rises when using CRF-40 as the compression factor, reaching 0.29 drop in AUC.\\

\indent We can conclude that re-compression can make the task of detecting synthetically generated videos more challenging and the higher the re-compression factor is the harder it is to accurately detect the synthetic video.
\indent To be able to accurately detect videos even after re-compression, one solution is to robust train our network against re-compression. In this process, we train the same detector with the same data with the only difference being the video frames have now been re-compressed with a multitude of compression factors.\\
\textbf{Robust Trainng Results.} As shown in table after testing the robust trained network the variation in performance going from non re-compressed frames to re-compressed frame shrinks significantly. For CRF-0 and CRF-10 the drop in AUC lowers from an average of 0.03 to 0.01, and for CRF-30 and CRF-40 where, respectively, we were seeing 0.13 and 0.29 drops in AUC now that number has changed to only 0.01 and 0.03 average drop in AUC across all generators.\\

\indent Based on the results of this experiment we can conclude that we can make our detectors invulnerable to re-compression artifacts by robust training them using a multitude of compression artifacts.

==> sec/old_or_temp/Det_Attrib_v2_Tai.tex <==
% Det_Attrib_v1

\section{Learning Synthetic Video Forensic Traces}
\label{sec:learn_synth_vid_traces}

As shown in Fig.~\ref{fig:trace_visualization}, forensic traces extracted from synthetic video generators are distinct from those made for image generation. Because of this, existing synthetic image detectors have a hard time detecting synthetic videos, as seen in our experiment in Sec.~\ref{sec:synth_img_det_on_videos}. However, in this section, we show that it is possible for existing synthetic image detectors to learn synthetic video's forensic traces through training. To do this, we present in the following sections the setup and results of three different experiments: Experiment 1 shows the synthetic video's detection performance of detectors which were retrained on synthetic video data; Experiment 2 shows the ability of these retrained detectors to attribute the source generator of synthetic videos; and Experiment 3 shows how different video compression strength affects the effectiveness of these detection systems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experimental Setup}
\label{subsec:common_exp_setup}

The following experiments all used the same experimental setup detailed here. 

\subheader{Data}
To train and evaluate the set of algorithms in these experiments, we collected a diverse set of real and synthetic videos. In total, we gathered \TODO{X} number of real videos (\TODO{X} frames) from the Moments in Time (MIT)~\citethis dataset and \TODO{X} videos (\TODO{X} frames) from the Video Authentication and Camera Identification Database (Video-ACID)~\citethis. To represent a wide variety of different generation architectures and techniques, we chose four popular sources of synthetic videos: Neural Radiance Fields videos from Luma AI (Luma)~\citethis, Transformer-based text-to-video generation algorithm from CogVideo~\citethis, Diffusion-based text-to-video generation algorithm from VideoCrafter-v1 (VC-v1)~\citethis, and Diffusion-based image-to-video generation method from Stable Video Diffusion (SVD)~\citethis. For each of these synthetic sources, we gathered enough videos to result in a total of \TODO{X} frames. 

To form the set of training, validation and testing videos we split the set of videos from each data sources into disjoint sets in which the proportion are approximately \TODO{X - X - X}, respectively.

More details are provided in Tab.~\ref{tab:video_dataset_stats}. 

\subheader{Metrics}
In the following experiments, we report the patch-level Area Under the Curve (AUC) detection performance for all approaches. 
\TODO{Put frame-level here if we have those results}
Additionally, we also fixed the patch size of all detectors to 256 x 256 pixels to ensure a fair comparison.

\subheader{Benchmarking Methods}
In experiment 1, we selected 6 state-of-the-art synthetic image detection approaches to retrain on our real \& synthetic video dataset. 
% To avoid confusion of what these systems are used to detect, we will refer to these systems only as "detectors" from now on. 
These detectors are:
1)\TODO{List paper name/author last name} ~\citethis, %MISLnet
2)\TODO{List paper name/author last name} ~\citethis, %ResNet-50
3)\TODO{List paper name/author last name} ~\citethis, %ResNet-34
4)\TODO{List paper name/author last name} ~\citethis, %Xception
5)\TODO{List paper name/author last name} ~\citethis, and %VGG-16
6)\TODO{List paper name/author last name} ~\citethis. %Inception-v2

\input{tables/video_dataset_stats_v0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Experiment 1: Synthetic Video Detection}
\label{subsec:exp1_synth_vid_det}

This experiment shows the synthetic video detection performance of existing synthetic image detectors when retrained on synthetic video data. To produce results shown in Tab.~\ref{tab:exp1_synth_vid_det}, we first trained each detection systems listed above on the training portion of our video dataset to produce binary classification decisions (real or synthetic), using the Cross-Entropy Loss function. Then, we evaluated each system's patch-level detection performance using AUC on test videos from individual generation methods in our dataset. Additionally, we also reported the overall average AUC over all generation methods.

From Tab.~\ref{tab:exp1_synth_vid_det}'s results, all image detectors received a significant boost in detection AUC when they are allowed to learn forensic traces from real and synthetic videos. In particular, \TODO{MISLnet}'s average detection AUC gained \TODO{X} (\TODO{from X to X}), and \TODO{ResNet-50}'s average detection AUC increased by 0.24 (from 0.70 to 0.94). This result suggests that authentic and synthetic video forensic traces are distinguishable, and that current synthetic image detectors' architecture can be used to adapt to detect synthetic videos.

\subsection{Experiment 2: Synthetic Video Source Attribution}
\label{subsec:exp2_synth_vid_attr}

In this experiment, we further show that learned forensic traces extracted from synthetic videos are not only effective in the detection task, but also viable to be used to attribute their source generation methods. To produce results shown in Tab.~\TODO{ref this table}, we trained each synthetic image detectors on the training portion of our video dataset to produce multi-classification decisions based on the number of possible generation methods in our training set, using the Cross-Entropy Loss function. Then, we evaluate each system's patch-level detection performance using AUC on test videos from individual generation methods in our dataset. 

Results from Tab.~\TODO{ref this table} shows that all current synthetic image detectors can be trained to achieve strong attribution capability. Notably....~\TODO{fill in when results are in}. 
These results suggest that different synthetic video generation architectures and algorithms leave behind distinct forensic traces that are highly-attributable and distinguishable from one another. This does not come as a surprise because as we have seen in Fig.~\ref{fig:trace_visualization} and in Sec.~\ref{sec:synth_video_traces}, these traces are unique to their source generator.

\subsection{Experiment 3: Effects of Video Compression Strength}
\label{subsec:exp3_vid_compression}

Prior works~\citethis have shown that different levels of compression strength impart different forensic traces upon the subjected media and make them harder to detect. 
Hence, to further evaluate the utility of synthetic video detectors when used to identify synthetic video in the wild, we performed a set of experiments showing the effects of varying video compression strengths on the performance of these detectors. We first tested the best performing network architecture in Experiment 1, MISLnet~\citethis, which has only seen training video data compressed at Compression Rate Factor (CRF) 23, on testing video data of 5 different CRFs, namely 0, 10, 20, 30, and 40. Results in Fig.~\TODO{ref fig} shows that this detector does well at CRF 20 but has a slight drop in performance on CRF 0 \& 10, and has a significant drop in performance on CRF 30 \& 40. This is because CRF 23 in training is the closest candidate to CRF 20 in testing. However, when we robustly trained this network with CRFs from 0 to 40, we see that MISLnet achieves high level of performance on across all benchmarking CRFs. This result suggests that while video compression strength negatively affects the performance of synthetic video detectors, it is possible to overcome this challenge with robust training using video data compressed at multiple compression strengths.


\begin{comment}
Videos can go through the process of re-compression for a multitude of reasons, when we upload a video to internet video sharing websites, in most cases,the video is recompressed with multiple re-compression factos. As demonstrated in ~\citethis, we know that compression artifacts can have a significant effect on the performance of detectors. When a video goes through the process of re-compression depending on the re-compression factor we may a range of difference in detector performance ranging from little to no difference to sizable performance drops in detector performance. \\
\indent To evaluate the robustness of our detector when it comes to re-compression we take the videos used to train the detector and recompress them with a range of compression factors.
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment was trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time~\citethis and VideoASID~\citethis and for synthetic videos we used videos from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment. All of the frames were also separately recompressed with factors ranging from CRF-0 to CRF-40\\
\textbf{Compression Effects Evaluation.}
As showcased in the table, different compression factors have different effects on the performance of the network. To summarize for lower compression factors such as CRF-0 and CRf-10 the effect on detector performance is minimal ranging from 0.01-0.04 drop in AUC.\\
\indent For CRF-20 we can almost see no effect on performance when we test the network trained on regular videos on videos recompressed with this compression factor which is to be expected since the default compression factor for videos is CRF-23 and CRF-20 is very close to that so the network is already familiar with the artifacts from this compression factor.\\
\indent In contrast, when we use CRF-30 and CRF-40 the effect on detector performance is significantly larger where when tested on videos recompressed with CRF-30 the network is on average has a 0.13 worse AUC across all generators and this number only rises when using CRF-40 as the compression factor, reaching 0.29 drop in AUC.\\

\indent We can conclude that re-compression can make the task of detecting synthetically generated videos more challenging and the higher the re-compression factor is the harder it is to accurately detect the synthetic video.
\indent To be able to accurately detect videos even after re-compression, one solution is to robust train our network against re-compression. In this process, we train the same detector with the same data with the only difference being the video frames have now been re-compressed with a multitude of compression factors.\\
\textbf{Robust Trainng Results.} As shown in table after testing the robust trained network the variation in performance going from non re-compressed frames to re-compressed frame shrinks significantly. For CRF-0 and CRF-10 the drop in AUC lowers from an average of 0.03 to 0.01, and for CRF-30 and CRF-40 where, respectively, we were seeing 0.13 and 0.29 drops in AUC now that number has changed to only 0.01 and 0.03 average drop in AUC across all generators.\\

\indent Based on the results of this experiment we can conclude that we can make our detectors invulnerable to re-compression artifacts by robust training them using a multitude of compression artifacts.
\end{comment}

==> sec/old_or_temp/Det_Attrib_v3DSV.tex <==
% Det_Attrib_v3DSV

\section{Learning Synthetic Video Forensic Traces}
\label{sec:learn_synth_vid_traces}




As shown in Fig.~\ref{fig:trace_visualization}, forensic traces extracted from synthetic video generators are distinct from those made for image generation. Because of this, existing synthetic image detectors have a hard time detecting synthetic videos, as seen in our experiments in Sec.~\ref{sec:synth_img_det_on_videos}. However, in this section, we show that it is possible for existing synthetic image detectors to learn synthetic video's forensic traces through training. To do this, we present in the following sections the setup and results of three different experiments: Experiment 1 shows the synthetic video's detection performance of detectors which were retrained on synthetic video data; Experiment 2 shows the ability of these retrained detectors to attribute the source generator of synthetic videos; and Experiment 3 shows how different video compression strengths affect the effectiveness of these detection systems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Experimental Setup}
\label{subsec:common_exp_setup}

The following experiments all used the same experimental setup detailed here. 

\subheader{Data}
To train and evaluate the set of algorithms in these experiments, we collected a diverse set of real and synthetic videos. In total, we used 5,313 number of real videos (108,000 frames) from the Moments in Time (MIT)~\cite{mit} dataset and 4,786 videos (108,000 frames) from the Video Authentication and Camera Identification Database (Video-ACID)~\cite{videoacid}. To represent a wide variety of different generation architectures and techniques, we chose four popular sources of synthetic videos: Neural Radiance Fields videos from Luma AI (Luma)~\cite{Luma}, Transformer-based text-to-video generation algorithm from CogVideo~\cite{cogvideo}, Diffusion-based text-to-video generation algorithm from VideoCrafter-v1 (VC-v1)~\cite{videocrafter1}, and Diffusion-based image-to-video generation method from Stable Video Diffusion (SVD)~\cite{stablevideo}. For each of these synthetic sources, we gathered enough videos to result in a total of 40,000 frames. 

To form the set of training, validation and testing videos we split the set of videos from each data sources into disjoint sets, in which the proportion are approximately 74\%, 6\%, 20\%, respectively.
%
More details about our dataset are provided in Tab.~\ref{tab:video_dataset_stats}. 

\subheader{Metrics}
In the following experiments, we report the patch-level Area Under the ROC Curve (AUC) detection performance for all approaches. 
\input{figures/video_auc}
\input{figures/video_rer}
Additionally, we also fixed the patch size of all detectors to 256 x 256 pixels to ensure a fair comparison.

\subheader{Benchmarking Methods}
In experiment 1, we selected 8 state-of-the-art synthetic image detection approaches to retrain on our real \& synthetic video dataset. 
% To avoid confusion of what these systems are used to detect, we will refer to these systems only as "detectors" from now on. 
These detectors are:

1) \TODO{List paper name/author last name} ~\citethis, %MISLnet

2) On the detection of synthetic images generated by diffusion models, Corvi et al. ~\cite{luisa}, %ResNet-50

3) Detecting and Simulating Artifacts in GAN Fake Images, Zhang et al. ~\cite{resnet34_method}, %ResNet-34

4) Locally GAN-generated face detection based on an improved Xception, Chen et al. ~\cite{xception_method}, %Xception

5) Detection, Attribution and Localization of GAN Generated
Images, Goebel et al. ~\cite{vgg16_method}, and %VGG-16

6) Detection of GAN-Generated Fake Images over Social Networks, Marra et al ~\cite{densenet_method}. %Densenet

7) Deep Image Fingerprint: Towards Low Budget Synthetic Image Detection and Model Lineage Analysis, Sinitsa et al. \cite{dif}

8) GenImage: A Million-Scale Benchmark for Detecting AI-Generated Image, Zhu et al. \cite{genimage}

\input{tables/video_dataset_stats_v1}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\subsection{Experiment 1: Synthetic Video Detection}
\label{subsec:exp1_synth_vid_det}

This experiment shows the synthetic video detection performance of existing synthetic image detectors when retrained on synthetic video data. To produce results shown in Tab.~\ref{tab:exp1_synth_vid_det}, we first trained each detection system listed above on the training portion of our synthetic video dataset to produce binary classification decisions (real or synthetic), using the Cross-Entropy Loss function. Then, we evaluated each system's patch-level detection performance using AUC on test videos from individual generation methods in our dataset. Additionally, we also reported the overall average AUC over all generation methods.

From Tab.~\ref{tab:exp1_synth_vid_det}'s results, all image detectors received a significant boost in detection AUC when they are allowed to learn forensic traces from real and synthetic videos. In particular,\TODO{who} MISLnet's\cite{bayar2016deep} average detection AUC gained 0.239 (from 0.744 to 0.983), and Corvi et al.(ResNet-50)'s average detection AUC increased by 0.24 (from 0.70 to 0.94). This result suggests that authentic and synthetic video forensic traces are distinguishable, and that current synthetic image detectors' architecture can be used to adapt to detect synthetic videos.

\input{tables/video_generator_table}

\subsection{Experiment 2: Synthetic Video Source Attribution}
\label{subsec:exp2_synth_vid_attr}

In this experiment, we further show that learned forensic traces extracted from synthetic videos are not only effective in the detection task, but also viable to be used to attribute their source generation methods. To produce results shown in Tab.\ref{tab:attribution}, we trained each synthetic image detectors on the training portion of our video dataset to produce multi-classification decisions based on the number of possible generation methods in our training set, using the Cross-Entropy Loss function. Then, we evaluate each system's patch-level detection performance using AUC on test videos from individual generation methods in our dataset. 
\input{tables/attribution_table}
Results from Tab.\ref{tab:attribution} shows that all current synthetic image detectors can be trained to achieve strong attribution capability. Notably MISLnet\cite{bayar2016deep} achieves an AUC of 0.991 when it comes to video source attribution across our four synthetic video generators. 
These results suggest that different synthetic video generation architectures and algorithms leave behind distinct forensic traces that are highly-attributable and distinguishable from one another. This does not come as a surprise because as we have seen in Fig.~\ref{fig:trace_visualization} and in Sec.~\ref{sec:synth_video_traces}, these traces are unique to their source generator.

\subsection{Experiment 3: Effects of Video Re-compression}
\label{subsec:exp3_vid_compression}

% Prior works~\citethis have shown that different levels of compression strength impart different forensic traces upon the subjected media and make them harder to detect. 
% Hence, to further evaluate the utility of synthetic video detectors when used to identify synthetic video in the wild, we performed a set of experiments showing the effects of varying video compression strengths on the performance of these detectors. We first tested the best performing network architecture in Experiment 1, MISLnet~\citethis, which has only seen training video data compressed at Compression Rate Factor (CRF) 23, on testing video data of 5 different CRFs, namely 0, 10, 20, 30, and 40. Results in Fig.~\ref{fig:crf_auc_plot} shows that this detector does well at CRF 20 but has a slight drop in performance on CRF 0 \& 10, and has a significant drop in performance on CRF 30 \& 40. This is because CRF 23 in training is the closest candidate to CRF 20 in testing. However, when we robustly trained this network with CRFs from 0 to 40, we see that MISLnet achieves high level of performance on across all benchmarking CRFs. This result suggests that while video compression strength negatively affects the performance of synthetic video detectors, it is possible to overcome this challenge with robust training using video data compressed at multiple compression strengths.

%%% added by danial to tai's edit %%%
Prior works~\citethis have shown that different levels of compression strength impart different forensic traces upon the subjected media and make them harder to detect. 
Hence, to further evaluate the utility of synthetic video detectors when used to identify synthetic video in the wild, we performed a set of experiments showing the effects of varying video compression strengths on the performance of these detectors.

Furthermore, as we can see in ~\ref{fig:crf_auc_plot}, the average AUC over our 4 video generators shifts depending on the CRF used for re-compression.in lower CRFs such as 0 and 10 the impact on performance is minimal as they do not impact the video severely and there is little to no reduction in performance for CRF-20 as it is close to the default CRF used for most systems which is CRF-23. However, for higher CRFs we can see that the average AUC drops significantly depending on the strength of the re-compression process and that is where robust training has the most impact. After robust training the same network with re-compressed images the detector is able to perform exceptionally better when faced with re-compressed videos as shown in the figure.

\subsection{Experiment 4: Video Level Performance Analysis}
\label{subsec:exp4_vid_level_analysis}
Although synthetic video detection can be very similar to synthetic image detection, an important aspect of video analysis is leveraging the temporal aspect of videos. 

In order to do so, we perform a video-level analysis of our chosen detector, leveraging multiple patches at the same time, as opposed to frame-level analysis using a single patch that we were using before.
If we consider an frame as $X_k$ where $X$ is the frame and $k$ represents the number of the frame in the sequence of frames for the video we can represent the image as an embedding using $\psi(X_k) = Z_k$ afterwards we can take the cumulative embedding as $ Z= \sum_{l=1}^N z_l$ where $N$ represents the number of patches used for analysis. Therefore, we can make the decision based on multiple patches rather than a single patch and leverage the temporal information provided by the video.

As seen in Fig.\ref{fig:video_auc_plot}, using higher number of patches for decision making allows us to improve our detection AUC. More specifically, for a detector trained on non-compressed video frames from the four generators used in this paper, we can see the AUC increasing by 0.013 reaching 0.995. Moreover, when we use the same detector robust trained on CRF-40 re-compressed frames we see a 0.031 increase in AUC reaching 0.984 from 0.953.

If we analyze our performance using relative error reduction,RER, as demonstrated in Fig.\ref{fig:video_rer_plot} we can see a similar pattern of error reduction for detectors trained on non-compressed video frames and robust-trained using CRF-40 compressed frames increasing the RER reaching 0.72 and 0.66, respectively.

In conclusion, video level analysis allows us to leverage the inherent traits of the video modality and as a result we are able to increase our performance by a significant degree.This could be specially beneficial for detecting re-compressed videos with a higher level of confidence.


\begin{comment}
Videos can go through the process of re-compression for a multitude of reasons, when we upload a video to internet video sharing websites, in most cases,the video is recompressed with multiple re-compression factos. As demonstrated in ~\citethis, we know that compression artifacts can have a significant effect on the performance of detectors. When a video goes through the process of re-compression depending on the re-compression factor we may a range of difference in detector performance ranging from little to no difference to sizable performance drops in detector performance. \\
\indent To evaluate the robustness of our detector when it comes to re-compression we take the videos used to train the detector and recompress them with a range of compression factors.
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment was trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time~\citethis and VideoASID~\citethis and for synthetic videos we used videos from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment. All of the frames were also separately recompressed with factors ranging from CRF-0 to CRF-40\\
\textbf{Compression Effects Evaluation.}
As showcased in the table, different compression factors have different effects on the performance of the network. To summarize for lower compression factors such as CRF-0 and CRf-10 the effect on detector performance is minimal ranging from 0.01-0.04 drop in AUC.\\
\indent For CRF-20 we can almost see no effect on performance when we test the network trained on regular videos on videos recompressed with this compression factor which is to be expected since the default compression factor for videos is CRF-23 and CRF-20 is very close to that so the network is already familiar with the artifacts from this compression factor.\\
\indent In contrast, when we use CRF-30 and CRF-40 the effect on detector performance is significantly larger where when tested on videos recompressed with CRF-30 the network is on average has a 0.13 worse AUC across all generators and this number only rises when using CRF-40 as the compression factor, reaching 0.29 drop in AUC.\\

\indent We can conclude that re-compression can make the task of detecting synthetically generated videos more challenging and the higher the re-compression factor is the harder it is to accurately detect the synthetic video.
\indent To be able to accurately detect videos even after re-compression, one solution is to robust train our network against re-compression. In this process, we train the same detector with the same data with the only difference being the video frames have now been re-compressed with a multitude of compression factors.\\
\textbf{Robust Trainng Results.} As shown in table after testing the robust trained network the variation in performance going from non re-compressed frames to re-compressed frame shrinks significantly. For CRF-0 and CRF-10 the drop in AUC lowers from an average of 0.03 to 0.01, and for CRF-30 and CRF-40 where, respectively, we were seeing 0.13 and 0.29 drops in AUC now that number has changed to only 0.01 and 0.03 average drop in AUC across all generators.\\

\indent Based on the results of this experiment we can conclude that we can make our detectors invulnerable to re-compression artifacts by robust training them using a multitude of compression artifacts.
\end{comment}

==> sec/old_or_temp/Det_Attrib_v4_MCS.tex <==
% Det_Attrib_v4_MCS

\section{Learning Synthetic Video Forensic Traces}
\label{sec:learn_synth_vid_traces}

%Results presented in Section~\ref{ } demonstrate that synthetic image detectors

Results presented in the previous two sections show that the traces left by synthetic video generators are different than those left by image generators, and that synthetic image detectors do not reliably detect these traces.

In this section, however, we show that synthetic video traces can be learned.  Through a series of experiments, we show that CNNs can be trained to accurately perform synthetic video detection and generator source attribution.   
Furthermore, we demonstrate that robust training can make these detectors perform strongly even in the presence of H.264 re-compression.  Additionally, we show how video-level detection can be performed to boost performance over frame-level detection.


%As shown in Fig.~\ref{fig:trace_visualization}, forensic traces extracted from synthetic video generators are distinct from those made for image generation. Because of this, existing synthetic image detectors have a hard time detecting synthetic videos, as seen in our experiments in Sec.~\ref{sec:synth_img_det_on_videos}. However, in this section, we show that it is possible for existing synthetic image detectors to learn synthetic video's forensic traces through training. To do this, we present in the following sections the setup and results of three different experiments: Experiment 1 shows the synthetic video's detection performance of detectors which were retrained on synthetic video data; Experiment 2 shows the ability of these retrained detectors to attribute the source generator of synthetic videos; and Experiment 3 shows how different video compression strengths affect the effectiveness of these detection systems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




\subsection{Experimental Setup}
\label{subsec:common_video_exp_setup}

\input{tables/video_dataset_stats_v1}

The following experiments all used the same experimental setup detailed here. 

\subheader{Video Training Data}
To train synthetic video detection systems in the following experiments, we collected a diverse set of real and synthetic videos. 

For the set of real videos, we gathered videos from both the Moments in Time (MIT)~\cite{mit} dataset and the Video Authentication and Camera Identification Database (Video-ACID)~\cite{videoacid}. Videos in the MIT dataset have much greater scene and content diversity, while videos in the Video-ACID dataset have much higher resolution and all videos came directly from video cameras. 

For the set of synthetic videos, we used 4 publicly available video generators to generate a large dataset for both training and testing purposes. These generation methods are: Luma~\cite{Luma}, VideoCrafter-v1~\cite{videocrafter1}, CogVideo~\cite{cogvideo}, and Stable Video Diffusion~\cite{stablevideo}. 
To create the synthetic videos in our dataset, we utilized a common set of text prompts chosen to represent a diverse set of motions and scenes.  Videos created using Luma were gathered from publicly shared videos, and similarly chosen to represent a diverse set of contents and activities. 

Additionally, we note that all videos is by default compressed using H.264 at CRF 23 since raw video is essentially never produced by a camera or a generator.
In summary, for training, we obtained 160,000 frames from 7,654 authentic videos and 160,000 frames from 6,197 synthetic videos. More detailed are provided in Tab.~\ref{tab:video_dataset_stats}.

\subheader{Video Testing Data}
To form the set of testing videos used in the following experiments, we utilized the same collection and generation methodology as for our training data. However, we kept an exclusive set of testing prompts to only be used to create testing data. Regarding videos from Luma, we also gathered a disjoint set of videos, completely separate from those in the training set.

In summary, for testing, we obtained 40,000 frames from 1,661 authentic videos and 40,000 frames from 1,429 synthetic videos. More detailed are provided in Tab.~\ref{tab:video_dataset_stats}.

\subheader{Out-of-distribution Test-only Synthetic Videos}
In addition to our in-distribution video testing set, we also evaluated the performance of different detection algorithms on an out-of-distribution, test-only set of videos. The synthetic videos in this set is collected from three recently emerging generation methods: Sora~\cite{sora}, Pika~\cite{Pika}, and VideoCrafter-v2~\cite{videocrafter2}. More details on this dataset are provided in Tab.~\ref{tab:ood_dataset_stats}

\subheader{Metrics}
In the following experiments, the performance of each detector was measured using the area under its ROC curve (AUC). In addition, to highlight performance differences, we calculated the Relative Error Reduction (RER) for the third experiment (Sec.~\ref{subsec:exp3_vid_compression}) and the fourth experiment (Sec.~\ref{subsec:exp4_vid_level_analysis}) below.


\subheader{Detectors}
To demonstrate the performance of different detection methods on detecting synthetic videos, we conducted our experiments with the diverse set of detectors listed in Sec.~\ref{subsec:synth_img_exp_setup} and in Tab.~\ref{tab:list_of_detectors}.

\begin{comment}
In the first experiment (details in Sec.~\ref{subsec:exp1_synth_vid_det}, we selected 8 state-of-the-art synthetic image detection approaches to retrain on our real \& synthetic video dataset. 
These detectors are:
1) \TODO{List paper name/author last name} ~\citethis, %MISLnet
2) On the detection of synthetic images generated by diffusion models, Corvi et al. ~\cite{luisa}, %ResNet-50
3) Detecting and Simulating Artifacts in GAN Fake Images, Zhang et al. ~\cite{resnet34_method}, %ResNet-34
4) Locally GAN-generated face detection based on an improved Xception, Chen et al. ~\cite{xception_method}, %Xception
5) Detection, Attribution and Localization of GAN Generated
Images, Goebel et al. ~\cite{vgg16_method}, and %VGG-16
6) Detection of GAN-Generated Fake Images over Social Networks, Marra et al ~\cite{densenet_method}. %Densenet
7) Deep Image Fingerprint: Towards Low Budget Synthetic Image Detection and Model Lineage Analysis, Sinitsa et al. \cite{dif}
8) GenImage: A Million-Scale Benchmark for Detecting AI-Generated Image, Zhu et al. \cite{genimage}
\end{comment}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%\subsection{Experiment 1: Synthetic Video Detection}
\subsection{Synthetic Video Detection}
\label{subsec:exp1_synth_vid_det}

First, we conducted an experiment in which we trained each candidate detector network to perform synthetic video detection using the training dataset describe above. We then evaluated their ability to detect each of the four synthetic video generators in the test set.  These experiments were carried out at a patch-level, i.e. all detection decisions were obtained using one patch taken from a single video frame.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                 %
%  Patch-Level Detection Results  %
%                                 %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{tables/exp1_synth_vid_det_v0}


%%%%%%%%%%%%%%%%%%%%%%%%%%
%                        %
%  Recompression Figure  %
%                        %
%%%%%%%%%%%%%%%%%%%%%%%%%%






The results of this experiment are presented in Table~\ref{tab:exp1_synth_vid_det}.  These results clearly show that synthetic videos can be reliably detected using each of these detectors.  All detectors evaluated achieved an average AUC of at least 0.93.  MISLnet achieved the highest average AUC of 0.982 and maintained consistently strong detection performance for each video generator.  
%
We note that each detector trained on synthetic video experienced an improvement of at least 0.23 in average AUC of when compared to its that was robustly trained on synthetic images.  
%
This further reinforces that synthetic video traces can be learned by existing architectures used for synthetic image detection. 

%that authentic and synthetic video forensic traces are distinguishable, and that current synthetic image detectors' architecture can be used to adapt to detect synthetic videos.


%This experiment shows the synthetic video detection performance of existing synthetic image detectors when retrained on synthetic video data. To produce results shown in Tab.~\ref{tab:exp1_synth_vid_det}, we first trained each detection system listed above on the training portion of our synthetic video dataset to produce binary classification decisions (real or synthetic), using the Cross-Entropy Loss function. Then, we evaluated each system's patch-level detection performance using AUC on test videos from individual generation methods in our dataset. Additionally, we also reported the overall average AUC over all generation methods.

%From Tab.~\ref{tab:exp1_synth_vid_det}'s results, all image detectors received a significant boost in detection AUC when they are allowed to learn forensic traces from real and synthetic videos. In particular,\TODO{who} MISLnet's\cite{bayar2016deep} average detection AUC gained 0.239 (from 0.744 to 0.983), and Corvi et al.(ResNet-50)'s average detection AUC increased by 0.24 (from 0.70 to 0.94). This result suggests that authentic and synthetic video forensic traces are distinguishable, and that current synthetic image detectors' architecture can be used to adapt to detect synthetic videos.



%\subsection{Experiment 2: Synthetic Video Source Attribution}
\subsection{Synthetic Video Source Attribution}
\label{subsec:exp2_synth_vid_attr}

Next, we conducted an experiment in which we evaluated each  network's ability to perform source attribution.  In this scenario, the forensic network must identify a video's source generator (or determine that the video is real). To adapt each network for this multi-class classification problem, we replaced its final layer with one containing multiple neurons, one for each generator along with an additional neuron for real.  Each network was trained to minimize the cross entropy between its soft-maxed output and a one hot vector identifying the true video source.  The trained network's AUC was assessed using the one-vs-the-rest strategy, i.e. any incorrect source attribution was counted as a miss irrespective of the class.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                              %
%  Source Attribution Results  %
%                              %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{tables/exp2_synth_vid_attr_v0}




The results of this experiment are shown in Table \ref{tab:exp2_synth_vid_attr}.  From these results, we can see that 
all networks achieved an AUC of at least 0.91, with most achieving an AUC of 0.95 or higher.  Again, the best performing network was MISLnet, which acheived an AUC of 0.991.
These results indicate that existing networks can be trained to perform accurate synthetic video source attribution.  We note that this result makes sense in light of the synthetic video traces visualized in Fig.~\ref{fig:trace_visualization}.  As discussed in Sec.~\ref{sec:synth_video_traces}, videos are generated using a wide variety of generation strategies and generator architectures.  As a result, there are often significant differenes between the traces left by each generator.  This makes it much easier for networks to accurately discriminate between each generator.



%\subsection{Experiment 3: Effects of Video Recompression}
\subsection{Effect of H.264 Recompression}
\label{subsec:exp3_vid_compression}
%and Robust Training}

\input{figures/exp3_recompression}


As we discussed in Sec.~\ref{sec:synth_img_det_on_videos}, it is well known that recompression can significantly reduce the performance of a forensic system.  
%
This is particularly important since recompression is often utized by social media platforms.  
%
In light of this, we conducted a set of experiments to understand the effect of H.264 compression on detection performance.  Additionally, we conducted experiments to assess the ability of robust training to mitigate these effects.  %Due to space constraints, we conducted this 
%Results are reported for the MISLnet detector
In light of space constraints, results are reported for the MISLnet detector, which achieved the highest detection and attribution performance in the previous experiments.

To carry out these experiments, we recompressed each video in the testing set with constant rate factors (CRFs) ranging from 0 (weak) to 40 (strong) in increments of 10. We note that videos are all initially H.264 compressed by either the camera that captured them or the system that generated them.  Typically, this is done using a default CRF of 23 or similar value. 
We then recompressed each video in the training set using the same CRF levels, then robustly trained MISLnet to perform synthetic video detection using this data.
%each detector using this recomrpessed data.
After this, we evaluated the performance of both the non-robustly trained and robustly trained version of this detector.

The results of this experiment are displayed in Fig.~\ref{fig:exp3_recompression}, which shows the AUC achieved by the detector at each CRF both with and without robust training.  
% 
From these results, we can see that without robust training, the detector's performance decreases as the CRF increases.  The notable exception to this is at CRF 20, which is close to the typical default CRF of 23.  Performance increases here because the CRF used during recompression is close to the default CRF that has already been seen during training.  

The results presented in Fig.~\ref{fig:exp3_recompression} also show that when robust training is utilized, the detector's performance remains consistently strong across all CRFs.
%These results also show that when robust training is utilized, the detector's performance remains fairly steady across all CRFs.  
Specifically, the detector is able to achieve an AUC of 0.95 or higher for all CRFs.  Furthermore, when the CRF is greater than or equal to 30, the detector is able to achieve an AUC of 0.97 or higher.  These results show that robust training can enable accurate synthetic video detection even after a video has been recompressed.  

%. Additionally, to show that it is possible to be robust to video compression, we also fine-tuned this network on re-compressed training videos at CRFs listed above and tested this version on our re-compressed video testing set.




  
%\subsection{Experiment 4: Video Level Performance Analysis}
\subsection{Video-Level Detection Performance}
\label{subsec:exp4_vid_level_analysis}


\input{figures/exp3_video_level_rer}
%One way in which synthetic video detection differs from synthetic image detection  

%Unlike their image counterparts, synthetic videos 

Unlike synthetic images, synthetic videos consist of a sequence of AI-generated frames.  %As a result, detection can be performed at a video-level by collecting information 
Because of this, generator traces are distributed temporally throughout a video.  This information can be exploited to perform detection at a video-level with greater accuracy.  


%To perform video-level detection, we first form a patch-level embedder $\psi(\cdot)$ by discarding the final layer of a synthetic video detector, and using the pre-softmax activations of this network as a patch-level embedding $z_k$. %z_k= \phi(x_k)$. 

To perform video-level detection, we first form a patch-level embedder $\psi(\cdot)$ by discarding the final layer of a pre-trained patch-level synthetic video detector.  The pre-softmax activations produced by this network corresond to patch-level embeddings that capture video generator traces. 
Next, a sequence of $N$ temporally distributed patches $x_k$ are gathered throughout a video and added together to form a single video-level embedding.  This is then passed through a softmax layer to produce the final output detection score $\delta$ such that
\begin{equation}
    \delta= \sigma\Bigl( \sum\nolimits_{k=1}^N \psi(x_k) \Bigr),
\end{equation}
where $\sigma(\cdot)$ is the softmax function.

%We conducted a set of experiments where we evaluated the performance of performing video-level detection using different numbers of patches taken throughout the video.

We conducted a series of experiments where we measured the performance of this video-level detection strategy using different numbers of patches.  In these experiments, we used the MISLnet detector architecture since it achieved the best performance for patch-level detection and attribution.   
Performance in terms of AUC was measured on both our non-recompressed testing set, as well as on a version of the testing set that was recompressed with a CRF of 40 for different numbers of patches $N$ ranging from 1 to 80.  Additionally, the percentage of relative error reduction (RER) over a patch-level detector was also calculated for each $N$.
%Performance was measured on both our non-recompressed testing set, as well as on a version of the testing set that was recompressed with a CRF of 40.




The results of these experiments are displayed in Fig.~\ref{fig:video_auc_plot} which shows video-level detection AUC vs number of patches used for detection, and in Fig.~\ref{fig:video_rer_plot} which shows the RER vs. number of patches used for detection.  
%
From these figures, we can see that performance increases as more patches are used to perform video-level detection.  
This is particularly strong for recompressed video, where the AUC grows from 0.953 to 0.984 as 80 patches are used.  This corresponds to a RER of 66\% over the patch-level detector.  We note that performance gains slow, however, after $N$ increases beyond 40.  
%
%These results show that important performance gains can be achieved by leverag the additional
These results show that video-level detection can achieve important performance gains by leveraging traces throughout an entire video.

We also note that while the increase in AUC for non-recompressed videos is not large in absolute terms, the RER achieved is substantial.  Specifically, when 80 patches are used, the video-level detector achieves an RER of $72.2\%$ over the patch-level detector. 
This is particularly important when performing synthetic video detection at scale, such as if a social media company were to examine all videos uploaded to its service.  Because of the large total number of videos examined, small gains in performance can correspond to a large reduction in the total number of false alarms.


%We note that while that AUC for non-recompressed videos does not increase a 


%To demonstrate this, we conducted a series of experiments in which we compared the performance of video-level detection to patch-level detection




\input{figures/exp3_video_level_auc}
%\hrulefill

\begin{comment}

Although synthetic video detection can be very similar to synthetic image detection, an important aspect of video analysis is leveraging the temporal aspect of videos. 

In order to do so, we perform a video-level analysis of our chosen detector, leveraging multiple patches at the same time, as opposed to frame-level analysis using a single patch that we were using before.
If we consider an frame as $X_k$ where $X$ is the frame and $k$ represents the number of the frame in the sequence of frames for the video we can represent the image as an embedding using $\psi(X_k) = Z_k$ afterwards we can take the cumulative embedding as $ Z= \sum_{l=1}^N z_l$ where $N$ represents the number of patches used for analysis. Therefore, we can make the decision based on multiple patches rather than a single patch and leverage the temporal information provided by the video.

As seen in Fig.\ref{fig:video_auc_plot}, using higher number of patches for decision making allows us to improve our detection AUC. More specifically, for a detector trained on non-compressed video frames from the four generators used in this paper, we can see the AUC increasing by 0.013 reaching 0.995. Moreover, when we use the same detector robust trained on CRF-40 re-compressed frames we see a 0.031 increase in AUC reaching 0.984 from 0.953.

If we analyze our performance using relative error reduction,RER, as demonstrated in Fig.\ref{fig:video_rer_plot} we can see a similar pattern of error reduction for detectors trained on non-compressed video frames and robust-trained using CRF-40 compressed frames increasing the RER reaching 0.72 and 0.66, respectively.

In conclusion, video level analysis allows us to leverage the inherent traits of the video modality and as a result we are able to increase our performance by a significant degree.This could be specially beneficial for detecting re-compressed videos with a higher level of confidence.



\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%






\begin{comment}
Videos can go through the process of re-compression for a multitude of reasons, when we upload a video to internet video sharing websites, in most cases,the video is recompressed with multiple re-compression factos. As demonstrated in ~\citethis, we know that compression artifacts can have a significant effect on the performance of detectors. When a video goes through the process of re-compression depending on the re-compression factor we may a range of difference in detector performance ranging from little to no difference to sizable performance drops in detector performance. \\
\indent To evaluate the robustness of our detector when it comes to re-compression we take the videos used to train the detector and recompress them with a range of compression factors.
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment was trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time~\citethis and VideoASID~\citethis and for synthetic videos we used videos from CogVideo~\citethis,VideoCrafter~\citethis, Stable Video Diffusion~\citethis and Luma ~\citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment. All of the frames were also separately recompressed with factors ranging from CRF-0 to CRF-40\\
\textbf{Compression Effects Evaluation.}
As showcased in the table, different compression factors have different effects on the performance of the network. To summarize for lower compression factors such as CRF-0 and CRf-10 the effect on detector performance is minimal ranging from 0.01-0.04 drop in AUC.\\
\indent For CRF-20 we can almost see no effect on performance when we test the network trained on regular videos on videos recompressed with this compression factor which is to be expected since the default compression factor for videos is CRF-23 and CRF-20 is very close to that so the network is already familiar with the artifacts from this compression factor.\\
\indent In contrast, when we use CRF-30 and CRF-40 the effect on detector performance is significantly larger where when tested on videos recompressed with CRF-30 the network is on average has a 0.13 worse AUC across all generators and this number only rises when using CRF-40 as the compression factor, reaching 0.29 drop in AUC.\\

\indent We can conclude that re-compression can make the task of detecting synthetically generated videos more challenging and the higher the re-compression factor is the harder it is to accurately detect the synthetic video.
\indent To be able to accurately detect videos even after re-compression, one solution is to robust train our network against re-compression. In this process, we train the same detector with the same data with the only difference being the video frames have now been re-compressed with a multitude of compression factors.\\
\textbf{Robust Trainng Results.} As shown in table after testing the robust trained network the variation in performance going from non re-compressed frames to re-compressed frame shrinks significantly. For CRF-0 and CRF-10 the drop in AUC lowers from an average of 0.03 to 0.01, and for CRF-30 and CRF-40 where, respectively, we were seeing 0.13 and 0.29 drops in AUC now that number has changed to only 0.01 and 0.03 average drop in AUC across all generators.\\

\indent Based on the results of this experiment we can conclude that we can make our detectors invulnerable to re-compression artifacts by robust training them using a multitude of compression artifacts.
\end{comment}

==> sec/old_or_temp/ImageDet_v1.tex <==
% ImageDet_v1

\section{Applying Synthetic Image Detectors To Video}

With the emergence of synthetic video generators recently, the need for a tools for detection of these videos has also emerged. It would be reasonable for one to assume that synthetic image detectors would be a good candidate for the job since a video is essentially a series of images orchestrated with temporal consistency. Consequently, we should be able to treat a single frame of the video as an image and use the synthetic image detectors to identify it. However, after investigating the synthetic image detectors for this function we find out that synthetic image detectors cannot successfully detect synthetic videos with an acceptable accuracy.

In addition, we have found the major cause of this lack of performance is not due to compression artifacts from the H.264 compression process. While it is scientifically established that the compression process can degrade the performance of detectors, it is also well-documented that robust training the detectors can significantly alleviate this issue for most detectors\citethis. In contrast, after our experiments we found that the boost of performance achieved from the process of robust training is insufficient to make synthetic image detectors a suitable candidate for this task.

To demonstrate this we designed and ran a set of experiments for evaluation of synthetic image detectors' ability to identify synthetic videos. For our experiments we utilize the following experimental procedures and data.

\subheader{Metrics}
AUC and accuracy.


\subheader{Training Data} 
The networks used in this experiment were trained using a dataset of real and synthetic images. Where for real images we used a subset of datasets COCO\citethis and LSUN\citethis and for synthetic images we used images from CycleGAN\citethis,StarGAN\citethis, StyleGAN2\citethis, StyleGAN3\citethis, ProGAN\citethis and Stable Diffusion\citethis taken from datasets in \citethis. We used 50,000 synthetic images and 50,000 real images for training in this experiment.

\subheader{Image Benchmarking data} 
The performance of the synthetic image detector network in detecting synthetic images accuractely was benchmarked using 10,000 synthetic images from CycleGAN\citethis,StarGAN\citethis, StyleGAN2\citethis, StyleGAN3\citethis, ProGAN\citethis and Stable Diffusion\citethis taken from datasets in \citethis and 10,000 real images from a subset of datasets COCO\citethis and LSUN\citethis.


\subheader{Detectors} 
For this experiment we use two set of detectors a set of networks trained on the same image dataset and evaluated on our video dataset and a set of pre-trained detectors that include resnet-50\citethis pretrained from \citethis DIF\citethis and Swin-T \citethis pretrained from \citethis. Moreover we re-train these detectors using the same image data used for non pre-trained networks to see the effect of training data on their performance.


\subheader{Evaluation Dataset} 
To measure the performance of the synthetic image detector on synthetic videos we use the frames of the videos generated by 4 different synthetic video generators , Luma\citethis, VideoCrafter\citethis, CogVideo\citethis, StableVideo Diffusion \citethis and real frames from subsets of the Moments in Time \citethis and Video-ASID\citethis datasets. We use 10,000 frames from each generator and 5000 frames from each real dataset totaling in 10,000 real frames for each experiment.


\subheader{Image-based Detector Evaluation} 
As we can see in Table 1, although the highest baseline accuracy for detecting images is 99.64\% using Xception net, when we try to apply the same detectors to video data we have a significant drop in performance where the best performance averaged over all generators is an AUC of 66.04\% and the highest overall is when we use vgg16\citethis to detect videos created by Luma\citethis at 67.03\%.

Moreover, we can observe in Table 2 that even after robust training the best average AUC improves by only 7.62\%  reaching an average best of 73.66\% and the best overall performance only reaches 75.46\% for when we use vgg16\citethis detect VideoCrafter\citethis. Based on this experiment we can deduce that compression degradation is not the only factor causing the drop in performance for synthetic detectors and we could come to the conclusion that the traces created by synthetic video generators must be inherently different than traces left behind by synthetic image generators.



==> sec/old_or_temp/ImageDet_v2_MCS.tex <==
% ImageDet_v2_MCS

%\section{Applying Synthetic Image Detectors To Video}
\section{Using Synthetic Image Detectors On Video}
\label{sec:synth_img_det_on_videos}

Given that video frames can be seen as a sequence of images, it is reasonable to expect that synthetic image detectors should be effective at detecting AI-generated synthetic videos. %However, our research has revealed an unexpected outcome: synthetic image detectors do not reliably detect synthetic videos. 
Surprisingly, however, we have found that synthetic image detectors do not successfully identify synthetic videos. 
Furthermore, we have found %determined 
that this issue is not primarily caused by the degradation of forensic traces due to H.264 video compression.

%To demonstrate the findings state above, 
To demonstrate these findings, we conducted a series of experiments in which we evaluated synthetic image detector's ability to detect synthetic videos.  
The details of these experiments ,as well as their outcomes, are presented below.

\subsection{Experimental Setup}
\label{ssec_ImDet_expSetup}

\subheader{Detectors} 
We evaluated the performance of multiple synthetic image detectors, including several well-known  detectors with publicly available implementations that were pre-trained by each detector's authors.  These include Corvi et al.'s ResNet-50-based approach \citethis, DIF \citethis, and Swin-T \citethis.  To augment these detectors, we implemented several additional detectors by training several well known CNNs to perform synthetic image detection, including ResNet-34~\citethis, VGG-16~\citethis, Xception~\citethis, DenseNet~\citethis.  
%
We note that the strategy of training a CNN to perform synthetic image detection is widely used throughout literature \citethis.


\subheader{Image Training Dataset} 
To train detectors that we implemented, we used a dataset of 100,000 images equally divided between real and synthetic.  For real images, we utilized a subset of the COCO dataset~\citethis and the LSUN dataset~\citethis, as was done in~\citethis.  For synthetic images, we used synthetic images from the datasets used in~\citethis consisting of images made by CycleGAN~\citethis, StarGAN~\citethis, StyleGAN2~\citethis, StyleGAN3~\citethis, ProGAN~\citethis, and Stable Diffusion~\citethis.

\subheader{Image Testing Dataset}
To benchmark the performance of each detector, we created a testing set of 20,000 images equally divided between real and synthetic.  This set was made by utilizing disjoint subsets of the datasets used to create the real and synthetic image training data.

\subheader{Video Testing Dataset}
To measure the performance of each detector, we created a testing dataset of both real and synthetically generated videos.  Synthetic videos were generated using four different publicly available video generators: Luma~\citethis, VideoCrafter~\citethis, CogVideo~\citethis, and StableVideo Diffusion~\citethis.  
%
Videos made using VideoCrafter~\citethis, CogVideo~\citethis, and StableVideo Diffusion~\citethis were created using a common set of text prompts chosen to represent a diverse set of content and motion.  Videos created using Luma were gathered from publicly shared videos, and similarly chosen to represent a diverse set of content and  motion. 
%
Real videos were taken equally from the Moments in Time (MiT)~\citethis and Video-ACID~\citethis datasets.  In total, our Video Testing Dataset consisted of 10,000 synthetic video frames from each generator, as well as 10,000 real video frames.

%\subheader{Evaluation Dataset} 
%To measure the performance of the synthetic image detector on synthetic videos we use the frames of the videos generated by 4 different synthetic video generators , Luma\citethis, VideoCrafter\citethis, CogVideo\citethis, StableVideo Diffusion \citethis and real frames from subsets of the Moments in Time \citethis and Video-ASID\citethis datasets. We use 10,000 frames from each generator and 5000 frames from each real dataset totaling in 10,000 real frames for each experiment.

\subheader{Metrics}  The performance of each detector was measured using the area under its ROC curve (AUC).


\subsection{Synthetic Image Detector Performance}


\input{tables/table_1_v0}
%\input{tables/table_2_v0}

%We evaluated the performance of each synthetic detector on our image testing dataset to establish their baseline performance.

%To establish the baseline performance of each synthetic image detector,  we evaluated the using our image testing dataset.
%we utilized our image testing dataset to compute its AUC. The results are presented in the second column of Table~\ref{tab:table_forsynth_im_noncompressed}. These baseline results show that when assessed on images, each detector can achieve strong performance.

We first evaluated the performance of each synthetic detector on our image testing dataset to establish their baseline performance.
These results are presented in the second column of Table~\ref{tab:synth_im_det_on_videos}.  All detectors but one achieved a baseline performance AUC of 0.90 or greater.  Furthermore, the majority of detectors achieved an AUC of 0.97 or greater.  The lowest baseline performance was for the pre-trained version of Swin-T with an AUC of 0.891, however this was increased to 0.911 after retraining using our image training dataset.  These baseline results verify that when assessed on images, each detector can achieve strong performance.

Next we evaluated each synthetic image detector using our video testing dataset.  These results are also shown in Table~\ref{tab:synth_im_det_on_videos}.
%
From these results, we can clearly see that all detectors experience substantial performance drops when evaluated on synthetic videos.  The highest average AUC achieved by any detector was 0.698, while the majority of detectors achieved an AUC of 0.65 or lower.  Furthermore, the drop in performance was not attributable to a single, difficult-to-detect generator.  AUCs achieved when testing each detector only on a  single generator did not vary substantially from the detector's mean performance.  In fact, detectors were unable to achieve AUCs higher than 0.7 for any single video generator in nearly all cases.

These results clearly show that synthetic image detectors experience substantial difficulty detecting synthetic videos.  This finding holds consistent across multiple different detector architectures, as well as when detectors are pre-trained by others or retrained using our dataset.

\subsection{Effect of H.264 Robust Training}
It is well known that compression alters forensic traces and can degrade a forensic detector's performance.  
%
Because of this, a plausible explanation for  synthetic image detector's the poor performance on synthetic video could be that H.264 video compression is degrading or altering synthetic video traces.

\input{tables/table_2_v0}


To test this hypothesis, we conducted an additional set of experiments in which each synthetic image detector was retrained to be robust against H.264 compression.  
%
Robust training involves augmenting the training dataset by recompressing all datapoints using different compression strengths, i.e. different quality factor for JPEG or different compression rate factors (CRFs) for H.264. 
%
It is well known that robust training can significantly mitigate the negative effects of compression.  As a result, if H.264 compression was truly the cause of a detector's low performance on synthetic video, we would expect the detector's performance to increase to a level much closer to its baseline performance after robust training.


Table~\ref{tab:synth_im_det_on_videos_h264} shows the performance of each synthetic image detector after it was robustly trained by augmenting the image training dataset with  H.264 compressed images using a CRF between 0 and 20.
%
The baseline detector performances on images in this table shows that robust training improves each detector's already strong performance on images.
%
Despite this, robust training did not substantially improve each detector's performance when evaluated on our video testing set.  The detector with the strongest performance on video after robust training was VGG-16, which obtained an AUC of 0.736 on video as opposed to its baseline performance of 0.993 on images.  Nearly all detectors acheived an average AUC below 0.70, with only the robustly trained versions of the Swin-T and VGG-16 detectors able to achieve a slightly higher performance.  Typically, robust training only improved the AUC of each detector by  \TODO{NUMBER} or less. The largest AUC gain was seen by \TODO{DETECTOR}, which only increased its AUC by  \TODO{DETECTOR} to  \TODO{DETECTOR}.


These results indicate that H.264 is not the primary cause of synthetic image detectors' poor performance when detecting synthetic videos.  Instead, the poor performance of synthetic image detectors after H.264 robust training suggests that a different factor is causing this phenomenon.





%As a result, we would expect that each detector's performance to increase to a level much closer to its baseline performance after robust training if H.264 compression was truly the cause of it's low performance on synthetic video.

%Robust training involves augmenting the training dataset by recompressing all datapoints using different compression strengths, i.e. different quality factor for JPEG or different constant rate factors (CRFs) for H.264.  Because prior work has shown that this can overcome the effects of compression or other similar post-processing operations, we would expect that if H.264 compression were the predominant causes o



%%%


%It is natural to assume that synthetic image detectors should detect AI-generated synthetic videos since each video frame can be viewed as an image.  
%Since the frames of a video can be viewed as a sequence of images, it is natural to assume that synthetic image detectors should detect AI-generated synthetic video. 
%Surprisingly, we have found that synthetic image detectors do not successfully identify synthetic videos.  

%In this section, we conduct a series 


%Furthermore, we have found that the cause of this is not predominantly due to forensic trace degradation caused by H.264 video compression.  While it is well known that compression alters forensic traces and can degrade a detectors performance, it is similarly well known that robust training on compressed data can significantly mitigate this negative effect.  As we will show, robustly training a synthetic image detector against video compression is insufficient to achieve comparable detection performance on synthetic video.  


==> sec/old_or_temp/ImageDet_v3_DSV.tex <==
% ImageDet_v2_MCS

%\section{Applying Synthetic Image Detectors To Video}
\section{Using Synthetic Image Detectors On Video}
\label{sec:synth_img_det_on_videos}

\input{tables/list_of_detectors}

Given that video frames can be seen as a sequence of images, it is reasonable to expect that synthetic image detectors should be effective at detecting AI-generated synthetic videos. %However, our research has revealed an unexpected outcome: synthetic image detectors do not reliably detect synthetic videos. 
Surprisingly, however, we have found that synthetic image detectors do not successfully identify synthetic videos. 
Furthermore, we have found %determined 
that this issue is not primarily caused by the degradation of forensic traces due to H.264 video compression.

%To demonstrate the findings state above, 
To demonstrate these findings, we conducted a series of experiments in which we evaluated synthetic image detector's ability to detect synthetic videos.  
The details of these experiments ,as well as their outcomes, are presented below.

\subsection{Experimental Setup}
\label{subsec:synth_img_exp_setup}

\subheader{Detectors} 
We evaluated the performance of a diverse set of detection algorithms. These include both publicly available pretrained detectors made specifically for synthetic image detection, and other architectures that are widely used to perform image forensic tasks. The complete list of these detectors and their referred-to names is provided in Tab.~\ref{tab:list_of_detectors}.

\begin{comment}
multiple synthetic image detectors, including several well-known  detectors with publicly available implementations that were pre-trained by each detector's authors.  These include Corvi et al.'s ResNet-50-based approach~\cite{luisa,resnet_archit}, DIF~\cite{dif}, and Swin-T~\cite{genimage,swint}.  To augment these detectors, we implemented several additional detectors by training several well known CNNs to perform synthetic image detection, including ResNet-34~\cite{resnet_archit,resnet34_method}, VGG-16~\cite{vgg16_method,vgg16_archit}, Xception~\cite{xception_method,xception_archit}, DenseNet~\cite{densenet_method,densenet_archit}.  
%
We note that the strategy of training a CNN to perform synthetic image detection is widely used throughout literature \citethis.
\end{comment}


\input{figures/synth_videos_gen}


\subheader{Image Training Dataset} 
To train detectors that we implemented, we used a dataset of 100,000 images equally divided between real and synthetic.  For real images, we utilized a subset of the COCO dataset~\cite{coco} and the LSUN dataset~\cite{lsun}, as was done in~\cite{luisa}.  For synthetic images, we used synthetic images from the datasets used in~\cite{openset} consisting of images made by CycleGAN~\cite{cyclegan}, StarGAN~\cite{stargan}, StyleGAN3~\cite{stylegan3}, ProGAN~\cite{progan}, and Stable Diffusion~\cite{stablediffusion}.

\subheader{Image Testing Dataset}
To benchmark the performance of each detector, we created a testing set of 20,000 images equally divided between real and synthetic.  This set was made by utilizing disjoint subsets of the datasets used to create the real and synthetic image training data.

\subheader{Video Testing Dataset}
To measure the performance of each detector, we created a testing dataset of both real and synthetically generated videos. 
%
Real videos were taken equally from the Moments in Time (MiT)~\cite{mit} and Video-ACID~\cite{videoacid} datasets.
%
Synthetic videos were generated using four different publicly available video generators: Luma~\cite{Luma}, VideoCrafter-v1~\cite{videocrafter1}, CogVideo~\cite{cogvideo}, and Stable Video Diffusion~\cite{stablevideo}.  
%
These synthetic videos were created using a common set of diversified content and motion text prompts, with the exception of videos from Luma, which were gathered from a similarly diverse set of publicly shared videos. 

In total, our video testing dataset consisted of 40,000 real video frames, as well as 40,000 synthetic frames, equally distributed among four generators. The qualitative samples of these videos are shown in Fig.~\ref{fig:video_gen_visualization}. Further details of this test set are provided in Tab.~\ref{tab:video_dataset_stats} and in Sec.~\ref{subsec:common_video_exp_setup} below.

%\subheader{Evaluation Dataset} 
%To measure the performance of the synthetic image detector on synthetic videos we use the frames of the videos generated by 4 different synthetic video generators , Luma\citethis, VideoCrafter\citethis, CogVideo\citethis, Stable Video Diffusion \citethis and real frames from subsets of the Moments in Time \citethis and Video-ASID\citethis datasets. We use 10,000 frames from each generator and 5000 frames from each real dataset totaling in 10,000 real frames for each experiment.

\subheader{Metrics}  The detection performance of each detector was measured using the area under its ROC curve (AUC).


\subsection{Synthetic Image Detector Performance}


\input{tables/exp1_synth_img_det_v0}
%\input{tables/table_2_v0}

%We evaluated the performance of each synthetic detector on our image testing dataset to establish their baseline performance.

%To establish the baseline performance of each synthetic image detector,  we evaluated the using our image testing dataset.
%we utilized our image testing dataset to compute its AUC. The results are presented in the second column of Table~\ref{tab:table_forsynth_im_noncompressed}. These baseline results show that when assessed on images, each detector can achieve strong performance.

We first evaluated the performance of each synthetic detector on our image testing dataset to establish their baseline performance.
These results are presented in the second column of Table~\ref{tab:synth_im_det_on_videos}.  All detectors but one achieved a baseline performance AUC of 0.90 or greater.  Furthermore, the majority of detectors achieved an AUC of 0.97 or greater.  The lowest baseline performance was for the pre-trained version of Swin-T with an AUC of 0.891, however this was increased to 0.911 after retraining using our image training dataset.  These baseline results verify that when assessed on images, each detector can achieve strong performance.

Next we evaluated each synthetic image detector using our video testing dataset.  These results are also shown in Table~\ref{tab:synth_im_det_on_videos}.
%
From these results, we can clearly see that all detectors experience substantial performance drops when evaluated on synthetic videos.  The highest average AUC achieved by any detector was 0.698, while the majority of detectors achieved an AUC of 0.65 or lower.  Furthermore, the drop in performance was not attributable to a single, difficult-to-detect generator.  AUCs achieved when testing each detector only on a  single generator did not vary substantially from the detector's mean performance.  In fact, detectors were unable to achieve AUCs higher than 0.7 for any single video generator in nearly all cases.

These results clearly show that synthetic image detectors experience substantial difficulty detecting synthetic videos.  This finding holds consistent across multiple different detector architectures, as well as when detectors are pre-trained by others or retrained using our dataset.

\subsection{Effect of H.264 Robust Training}
It is well known that compression alters forensic traces and can degrade a forensic detector's performance.  
%
Because of this, a plausible explanation for  synthetic image detector's the poor performance on synthetic video could be that H.264 video compression is degrading or altering synthetic video traces.

\input{tables/exp2_synth_img_h264_det_v0}


To test this hypothesis, we conducted an additional set of experiments in which each synthetic image detector was retrained to be robust against H.264 compression.  
%
Robust training involves augmenting the training dataset by recompressing all datapoints using different compression strengths, i.e. different quality factor for JPEG or different compression rate factors (CRFs) for H.264. 
%
It is well known that robust training can significantly mitigate the negative effects of compression~\citethis.  As a result, if H.264 compression was truly the cause of a detector's low performance on synthetic video, we would expect the detector's performance to increase to a level much closer to its baseline performance after robust training.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%                                %
%  SYNTHETIC VIDEO TRACE FIGURE  %
%                                %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{figures/trace_vis_v0}

Table~\ref{tab:synth_im_det_on_videos_h264} shows the performance of each synthetic image detector after it was robustly trained by augmenting the image training dataset with  H.264 compressed images using a CRF between 0 and 20.
%
The baseline detector performances on images in this table shows that robust training improves each detector's already strong performance on images.
%
Despite this, robust training did not substantially improve each detector's performance when evaluated on our video testing set.  The detector with the strongest performance on video after robust training was VGG-16, which obtained an AUC of 0.736 on video as opposed to its baseline performance of 0.993 on images.  Nearly all detectors acheived an average AUC below 0.70, with only the robustly trained versions of the Swin-T and VGG-16 detectors able to achieve a slightly higher performance.  On average, robust training only improved the AUC of each detector by 0.052. The largest AUC gain was seen by ResNet-34\cite{resnet34_method,resnet_archit}, which only increased its average AUC by 0.079 to 0.694.


These results indicate that H.264 is not the primary cause of synthetic image detectors' poor performance when detecting synthetic videos.  Instead, the poor performance of synthetic image detectors after H.264 robust training suggests that a different factor is causing this phenomenon.





%As a result, we would expect that each detector's performance to increase to a level much closer to its baseline performance after robust training if H.264 compression was truly the cause of it's low performance on synthetic video.

%Robust training involves augmenting the training dataset by recompressing all datapoints using different compression strengths, i.e. different quality factor for JPEG or different constant rate factors (CRFs) for H.264.  Because prior work has shown that this can overcome the effects of compression or other similar post-processing operations, we would expect that if H.264 compression were the predominant causes o



%%%


%It is natural to assume that synthetic image detectors should detect AI-generated synthetic videos since each video frame can be viewed as an image.  
%Since the frames of a video can be viewed as a sequence of images, it is natural to assume that synthetic image detectors should detect AI-generated synthetic video. 
%Surprisingly, we have found that synthetic image detectors do not successfully identify synthetic videos.  

%In this section, we conduct a series 


%Furthermore, we have found that the cause of this is not predominantly due to forensic trace degradation caused by H.264 video compression.  While it is well known that compression alters forensic traces and can degrade a detectors performance, it is similarly well known that robust training on compressed data can significantly mitigate this negative effect.  As we will show, robustly training a synthetic image detector against video compression is insufficient to achieve comparable detection performance on synthetic video.  


==> sec/old_or_temp/Learning_Synthetic_Video_Traces.tex <==
\subsection{Learning Synthetic Video Traces}
Knowing that different generators leave different traces behind we conduct experiments to learn each and all of these traces to be able to accurately detect synthetically generated videos. \\
\indent In synthetic image generators the network has significant upsampling traces left behind due to starting from an image and repeatedly up-sampled until the desired outcome has been achieved this is know to be especially the case for Generative Adversarial Networks\citethis. However, due to the drop in the performance of synthetic image detectors and the observation in the previous section it would be reasonable to assume that this is not the case for synthetic video generators.\\
\indent As a result, we use a multitude of forensic architectures to try and learn the traces left behind by the synthetic video generators where instead of training the detector on synthetic images we train the network using frames extracted from videos generated by different synthetic video generation methods.\\
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The networks used in this experiment were trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time\citethis and VideoASID\citethis and for synthetic videos we used videos from CogVideo\citethis,VideoCrafter\citethis, Stable Video Diffusion\citethis and Luma \citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment.\\
\textbf{Video Benchmarking data.} The performance of the synthetic video detector network in detecting synthetic videos accurately was benchmarked using 10,000 synthetic frames from each synthetic video generator from CogVideo\citethis,VideoCrafter\citethis, Stable Video Diffusion\citethis and Luma \citethis and 20,000 real video frames from a subset of datasets Moments in Time\citethis and VideoASID\citethis.\\
\textbf{Video-based Detector Evaluation.} As demonstrated in Table3, the same detectors used for detecting synthetic image when trained on synthetic video data can achieve the sufficient AUCs for accurate detection we can see the average AUC rising to 0.956 whereas when we used the same detectors trained on synthetic images the average AUC was only 0.704 even after robust training on recompressed data. In Addition, we observe that the best detector to be used for this cas is Mislnet\citethis with the testing AUC of 0.982 outperforming the other detectors by at least 0.012 under equal conditions. \\
\indent From this experriment we can deduce that although synthetically generated videos are not hard to detect the detectors still need to be trained on suitable data to learn the novel traces left behind by the synthetic video generators in order to be able to detect them with sufficient performance. 

==> sec/old_or_temp/Synthetic_Image_Detectors_in_Synthetic_Video_Detection.tex <==
\subsection{Synthetic Image Detectors in Synthetic Video Detection}
With the emergence of synthetic video generators recently, the need for a tools for detection of these videos has also emerged. It would be reasonable for one to assume that synthetic image detectors would be a good candidate for the job since a video is essentially a series of images orchestrated with temporal consistency. Consequently, we should be able to treat a single frame of the video as an image and use the synthetic image detectors to identify it. However, after investigating the synthetic image detectors for this function we find out that synthetic image detectors cannot successfully detect synthetic videos with an acceptable accuracy.\\
\indent In addition, we have found the major cause of this lack of performance is not due to compression artifacts from the H.264 compression process. While it is scientifically established that the compression process can degrade the performance of detectors, it is also well-documented that robust training the detectors can significantly alleviate this issue for most detectors\citethis. In contrast, after our experiments we found that the boost of performance achieved from the process of robust training is insufficient to make synthetic image detectors a suitable candidate for this task.\\
\indent To demonstrate this we designed and ran a set of experiments for evaluation of synthetic image detectors' ability to identify synthetic videos. For our experiments we utilize the following experimental procedures and data.
\\ \textbf{Metrics.} AUC and accuracy.\\ \textbf{Training Data.} The networks used in this experiment were trained using a dataset of real and synthetic images. Where for real images we used a subset of datasets COCO\citethis and LSUN\citethis and for synthetic images we used images from CycleGAN\citethis,StarGAN\citethis, StyleGAN2\citethis, StyleGAN3\citethis, ProGAN\citethis and Stable Diffusion\citethis taken from datasets in \citethis. We used 50,000 synthetic images and 50,000 real images for training in this experiment.\\ 
\textbf{Image Benchmarking data.} The performance of the synthetic image detector network in detecting synthetic images accuractely was benchmarked using 10,000 synthetic images from CycleGAN\citethis,StarGAN\citethis, StyleGAN2\citethis, StyleGAN3\citethis, ProGAN\citethis and Stable Diffusion\citethis taken from datasets in \citethis and 10,000 real images from a subset of datasets COCO\citethis and LSUN\citethis.\\
\textbf{Evaluation Dataset.} To measure the performance of the synthetic image detector on synthetic videos we use the frames of the videos generated by 4 different synthetic video generators , Luma\citethis, VideoCrafter\citethis, CogVideo\citethis, StableVideo Diffusion \citethis and real frames from subsets of the Moments in Time \citethis and Video-ASID\citethis datasets. We use 10,000 frames from each generator and 5000 frames from each real dataset totaling in 10,000 real frames for each experiment.\\
\textbf{Image-based Detector Evaluation.} As we can see in Table 1, although the highest baseline accuracy for detecting images is 99.64\% using Xception net, when we try to apply the same detectors to video data we have a significant drop in performance where the best performance averaged over all generators is an AUC of 66.04\% and the highest overall is when we use vgg16\citethis to detect videos created by Luma\citethis at 67.03\%.\\
\indent Moreover, we can observe in Table 2 that even after robust training the best average AUC improves by only 7.62\%  reaching an average best of 73.66\% and the best overall performance only reaches 75.46\% for when we use vgg16\citethis detect VideoCrafter\citethis. Based on this experiment we can deduce that compression degradation is not the only factor causing the drop in performance for synthetic detectors and we could come to the conclusion that the traces created by synthetic video generators must be inherently different than traces left behind by synthetic image generators.

==> sec/old_or_temp/Synthetic_Video_Source_Attribution.tex <==
\subsection{Synthetic Video Source Attribution}
While detection is the most important issue when it comes to synthetic videos, source attribution is of equal importance. Moreover, since the traces from different generators vary from one another significantly we can easily use a multi-class classifier to tackle the problem of source attribution.
\textbf{Metrics.} AUC\\
\textbf{Training Data.} The network used in this experiment were trained using a dataset of real frames from real videos and synthetic frames from synthetically generated videos. Where for real videos we used a subset of datasets Moments in Time\citethis and VideoASID\citethis and for synthetic videos we used videos from CogVideo\citethis,VideoCrafter\citethis, Stable Video Diffusion\citethis and Luma \citethis. We used 40,000 synthetic frames from each generator and 80,000 real frames from each real video dataset source for training in this experiment.\\
\textbf{Video Benchmarking data.} The performance of the synthetic video attribution network in detecting synthetic images accurately was benchmarked using 10,000 synthetic frames from each synthetic video generator from CogVideo\citethis,VideoCrafter\citethis, Stable Video Diffusion\citethis and Luma \citethis and 20,000 real video frames from a subset of datasets Moments in Time\citethis and VideoASID\citethis.\\
\textbf{Video Source Attribution Evaluation} As we can see in Table 5. using the same base architecture we used for detection and the same data and changing the task from binary classification, detection, to multi-class classification we are able to attribute each video to its source generator with a testing AUC of 0.985. This finding further solidifies the idea that synthetic video traces are not only distinct from synthetic image traces but are also significantly distinguishable from each other.

==> sec/old_or_temp/Synthetic_Video_Traces.tex <==
\section{Synthetic Video Traces}
Considering the findings of previous section, it would be reasonable to assume that synthetic video generators have significantly different forensic traces compared to synthetic image generators where even after eliminating the effects of video compression synthetic image detectors are not able to have sufficient performance when it comes to detecting synthetic videos.\\
\indent In order to have a qualitative demonstration of this claim we decided to visualize low-level synthetic image generator and video generator traces and compare them together. We do this using the same method used in \citethis where we use the de-noising network from \citethis to de-noise the synthetic image or frames of the synthetic video subtract them from the original and visualize the spectral analysis as demonstrated in \citethis. \\ 
\indent Figure 1, allows us to have a better understanding of the traces left behind by each generator, being synthetic image or video generator, we can see that the visualization of the traces from  ProGAN\citethis,  and StyleGAN3\citethis, StarGANM\citethis, CycleGAN\citethis have a significantly different shape from the visualization for Cogvideo\citethis and  Luma\citethis, sora \citethis, pika\citethis. However, the trace visualization from VideoCrafter \citethis is closely similar to the one from latent diffusion\citethis and interestingly although the trace visualization from Stable Image Diffusion v 1.9 \citethis is close to the trace visualization for Stable Video Diffusion\citethis created using the same images from Stable Image Diffusion v1.9 \citethis, in some areas they are distinguishable from each other for instance the traces from stable image diffusion are more densely populated around the x axis which would explain the drop in performance observed in synthetic image detectors.\\
\indent To delve deeper in this analysis, we observer regularly appearing dots in the synthetic image generators which can be attributed to the up-sampling operation traces commonly used in U-net style networks as demonstrated by \citethis. However, most synthetic video generators largely lack this structure.\\
\indent We know that synthetic video generators employ significantly different architectures compared to synthetic image generators and for that reason the pattern observer in their trace visualization is drastically different from one another. Moreover we see that different families of generators, depending if they use Diffusion models, Transformers, Neural Radiance Fields or a combination of those have significantly different traces we can see this point illustrated by comparing the visualizations from Sora \citethis and Luma \citethis that are ,respectively, Neural Radiance Field and combination based we can see that the visualization is significantly different from any other generator. 


==> sec/old_or_temp/experiments.tex <==
\section{Experiments}
\subsection{Dataset}
\subheader{Training and Evaluation Dataset}
Our experiment structure includes different modalities of data from a myriad of sources. In general the data is split into 80\% for training and 20\% for testing.
\\ \textbf{Video Dataset} The video dataset includes synthetic and real videos for our real videos we use Video-ASID \cite{videoasid} which includes videos shot by different camera models from different scenes and landscapes. In addition to Video-ASID we use the Moments in Time \cite{Mit} dataset that includes various videos of human motion gathered from a variety of sources over the web. \\ For the synthetic portion of our dataset we use different families of video synthesis techniques that include diffusion models, transformers and Neural Radiance Fields. In the diffusion model family we have VideoCrafter version 1 and 2 \cite{videocrafter} and Stable Video diffusion \cite{stablevideo} and for Neural Radiance fields and transformers we include CogVideo \cite{cogvideo} and Luma \cite{Luma} respectively. \\ \textbf{Testing Dataset} In addition to the 20\% of the training dataset allocated to testing, we included videos from other sources. We use Sora \cite{sora}, StableVideo version 2,1 \cite{stablevideo}, PikaLabs\cite{pikalabs} where all of them are from the diffusion model family. Using these generators for testing not only allows us to evaluate the transferability of the models we can demonstrate how we can improve models to be able to identify new generators using limited data.

\subsection{Synthetic Image Detector Evaluation} As established in previous sections we have had a rise in the emergence of synthetic image generators and recently researchers have discovered reliable methods for detecting images generated by these methods. Moreover, videos are essentially an ensemble of many frames come together in a temporally continuous manner. Hence, in this section we put some of the most recent and well known methods of detection to test against synthetic videos. In this experiment we have two sections one including commonly used architectures for classification and detection trained on synthetic images from cyclegan \cite{cyclegan}, progan \cite{progan}, stargan\cite{stargan}, stylegan2\cite{stylegan2}, stylegan3\cite{stylegan3} and for our real images we used COCO\cite{coco} and LSUN \cite{lsun} to replicate the training setup used in other detectors\cite{luisa} and test the transferability of that performance to videos we use our synthetic video evaluation dataset. We use 50 thousand synthetic images and 50 thousand real images for training and 10 thousand frames from synthetic videos and 10 thousand frames from real videos from the video dataset for testing.\\ As we can see in table 2, networks trained on synthetic images have astonishingly high performance when it comes to detecting synthetically generated images. However when we test the same networks on video frames the performance drops so significantly that the best performing network is DenseNet tested against StableVideo Diffusion with an AUC of 0.713.


\begin{table*}
	\caption{Networks trained on synthetic images and tested on synthetic video frames}
	\label{tab:table_forsynth_im_noncompressed}
	\centering
	\begin{tblr}{
			cells = {c},
			cell{1}{3} = {c=4}{},
			vline{2-4} = {1}{},
			vline{2-3,7} = {2-6}{},
			hline{2} = {-}{},
			hline{3} = {3-6}{},
		}
		Network  & Baseline Accuracy (Images) & Testing Accuracy (Videos) &          &                   &                       & Average Accuracy \\
		&                            & Luma                      & CogVideo & VideoCrafter      & StableVideo Diffusion &                  \\
		resnet34 & 98.30 \%                  & 57.64\%                   & 62.33 \% & 61.62 \%          & \textbf{64.71 \%}     & 61.57\%          \\
		vgg16    & 98.97 \%                   & 63.57\%                   & 65.20\%  & \textbf{68.43\%}  & 66.95\%               & \textbf{66.04\%} \\
		Xception & 99.64 \%                  & 59.24 \%                  & 63.80 \% & \textbf{67.03 \%} & 66.44 \%              & 64.13\%          \\
		DenseNet & 97.48 \%                   & 55.92 \%                  & 58.47 \% & 64.72 \%          & \textbf{67.81 \%}     & 62.41\%          
	\end{tblr}
\end{table*}

\begin{table*}[t] % Use table* to span both columns
	\caption{Networks trained on h.264 compressed synthetic Images tested on synthetic videos}
	\label{tab:your_table_label}
	\centering
	\begin{tblr}{
		cells = {c},
		cell{1}{3} = {c=4}{},
		vline{2-4} = {1}{},
		vline{2-3,7} = {2-6}{},
		hline{2} = {-}{},
		hline{3} = {3-6}{},
	}
	Network  & Baseline Accuracy (Images) & Testing Accuracy (Videos) &          &                   &                       & Average Accuracy \\
	&                            & Luma                      & CogVideo & VideoCrafter      & StableVideo Diffusion &                  \\
	resnet34 & 98.91 \%                  & 66.35\%                   & 68.74 \% & 70.04 \%          & \textbf{72.79 \%}     & 69.48\%          \\
	vgg16    & 99.30 \%                   & 71.90\%                   & 74.31\%  & \textbf{75.46\%}  & 72.98\%               & \textbf{73.66\%} \\
	Xception & 97.96 \%                  & 64.24 \%                  & 69.20 \% & \textbf{73.42 \%} & 70.84 \%              & 69.43\%          \\
	DenseNet & 99.53 \%                   & 63.71 \%                  & 65.87 \% & 71.55 \%          & \textbf{74.92 \%}     & 69.01\%          
	\end{tblr}
\end{table*}

\textbf{Pretrained Synthetic image detectors} To further evaluate the performance of established synthetic image detectors we picked three of the most recent and high performance synthetic image detectors\cite{Luisa,FID,thirdone} and used them to see if they can accurately detect a frame of a synthetically generated video. As shown in table 4 while some of the detectors do a better job than the others, when tested against the frames of synthetic videos the AUC of synthetic images doesn't go higher than 0.7 and in some cases the detector does not detect synthetic video frames at such is in the case of DIF \cite{DIF} we see that the detector is classifying synthetic video frames as real images and hence getting an AUC of 0.500.

\subsection{Network Architecture Evaluation}
\subsection{Video Compression Effects}
\subsection{Detection Transferability}

==> sec/old_or_temp/problem.tex <==
\section{Problem Formulation}
\input{sec/Synthetic_Image_Detectors_in_Synthetic_Video_Detection}
\input{tables/table_1}
\input{tables/table_2}
\input{tables/table_3}

\input{sec/Synthetic_Video_Traces}
\input{sec/Learning_Synthetic_Video_Traces}

\input{sec/Synthetic_Video_Source_Attribution}
\input{sec/Video_Compression_Effects}


==> tables/exp1_synth_vid_det_v0.tex <==
\begin{table}[!t]
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{32mm}m{12mm}m{16mm}m{14mm}m{9mm}m{14mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{2} = {c=5}{0.634\linewidth,c},
				vline{1-2, 6, 7} = {-}{},
				hline{1-3,6, 11} = {-}{},
			}
			\textbf{Method}   & \textbf{Videos} &  &  &  & \\
			  & \textbf{Luma} & \textbf{CogVideo} & \textbf{VC-v1} & \textbf{SVD} & \textbf{Average}\\
			ResNet-50~\cite{resnet_archit}  & 0.921 & \textbf{0.935} & 0.940 & 0.939 & 0.934 \\
			DIF~\cite{dif}  & 0.938 & 0.957 & 0.969 & 0.973 & 0.959 \\
			Swin-T~\cite{swint}  & 0.960 & 0.964 & 0.986 & 0.991 & 0.975 \\
            ResNet-34~\cite{resnet_archit}  & 0.916 & 0.930 & 0.942 & 0.951 & 0.935  \\
            VGG-16~\cite{vgg16_archit}  & 0.937 & 0.944 & 0.965 & 0.960 & 0.951  \\
            Xception~\cite{xception_archit}  & 0.928 & 0.951 & 0.973 & 0.969 & 0.955  \\
            DenseNet ~\cite{densenet_archit}  & 0.918 & 0.924 & 0.964 & 0.968 & 0.943  \\
            MISLnet ~\cite{openset}  & \textbf{0.975} & \textbf{0.980} & \textbf{0.991} & \textbf{0.987} & \textbf{0.983}  \\
		\end{tblr}
	}
    \caption{Detection performance of methods trained and tested on different synthetic video generation methods: Luma~\cite{Luma}, CogVideo~\cite{cogvideo}, VideoCrafter (VC-v1)~\cite{videocrafter1}, and Stable Video Diffusion (SVD)~\cite{stablevideo} Performance numbers are measured using AUC.}
    \label{tab:exp1_synth_vid_det}
\end{table}

==> tables/old_or_temp/recompression1.tex <==
\begin{table*}[!t]
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{22mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}},
				row{1-2} = {c},
				cell{1}{1} = {r=2}{},
				cell{1}{2} = {c=2}{0.168\linewidth,c},
				cell{1}{4} = {c=2}{0.168\linewidth,c},
				cell{1}{6} = {c=2}{0.168\linewidth,c},
				cell{1}{8} = {c=2}{0.168\linewidth,c},
				cell{1}{10} = {c=2}{0.168\linewidth,c},
				column{2-11} = {c},
				column{1} = {l},
				vlines,
				hline{1,3,7} = {-}{},
				hline{2} = {2-11}{},
			}
			\textbf{Generator } & \textbf{CRF 0} &  & \textbf{CRF 10} &  & \textbf{CRF 20} &  & \textbf{CRF 30} &  & \textbf{CRF 40} & \\
			& \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed}\\
			Luma~\citethis & 0.97 & 0.97 & 0.95 & 0.97 & 0.97 & 0.98 & 0.86 & 0.96 & 0.70 & 0.93\\
			CogVideo~\citethis & 0.96 & 0.98 & 0.92 & 0.97 & 0.98 & 0.98 & 0.82 & 0.98 & 0.67 & 0.95\\
			Vid.Crafter~\citethis & 0.95 & 0.98 & 0.94 & 0.96 & 0.98 & 0.99 & 0.85 & 0.98 & 0.69 & 0.95\\
			SVD~\citethis & 0.96 & 0.97 & 0.94 & 0.97 & 0.98 & 0.98 & 0.88 & 0.98 & 0.70 & 0.98
		\end{tblr}
	}
    \caption{Detection performance of MISLnet on different synthetic video generation methods at different Compression Rate Factors (CRF) and whether the video is recompressed. Performance numbers are measured in AUC.}
    \label{tab:exp3_compression_strength}
\end{table*}

==> tables/old_or_temp/table_3.tex <==
\begin{table}[!t]
	\centering
	\resizebox{0.8\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {Q[215]Q[333]Q[346]},
				column{2} = {c},
				column{3} = {c},
				vlines,
				hline{1-2,10} = {-}{},
			}
			 \textbf{Architecture} & \textbf{Average AUC}\\
              Corvi et al. & 0.944\\
              DIF & 0.961\\
              Swin-T & 0.979\\
              ResNet-34 & 0.937\\
              VGG-16 & 0.950\\
              Xception & 0.955\\
              DenseNet &0 .947 \\
			 MISLnet & \textbf{0.982}\\
		\end{tblr}
	}
    \caption{Average patch-level detection performance of different methods with different underlying network architectures on the set of testing videos gathered from all synthetic video generators used in this paper. These include: Luma~\citethis, CogVideo~\citethis, VideoCrafter~\citethis, and Stable Video Diffusion~\citethis. Performance numbers are measured using AUC.}
    \label{tab:exp1_synth_vid_det}
\end{table}

==> tables/recompression1.tex <==
\begin{table*}[!t]
	\centering
	\caption{Detection performance of MISLnet on different synthetic video generation methods at different Compression Rate Factors (CRF) and whether the video is recompressed. Performance numbers are measured in AUC.}
	\label{tab:exp3_compression_strength}
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{22mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}m{17.5mm}},
				row{1-2} = {c},
				cell{1}{1} = {r=2}{},
				cell{1}{2} = {c=2}{0.168\linewidth,c},
				cell{1}{4} = {c=2}{0.168\linewidth,c},
				cell{1}{6} = {c=2}{0.168\linewidth,c},
				cell{1}{8} = {c=2}{0.168\linewidth,c},
				cell{1}{10} = {c=2}{0.168\linewidth,c},
				column{2-11} = {c},
				column{1} = {l},
				vlines,
				hline{1,3,7} = {-}{},
				hline{2} = {2-11}{},
			}
			\textbf{Generator } & \textbf{CRF 0} &  & \textbf{CRF 10} &  & \textbf{CRF 20} &  & \textbf{CRF 30} &  & \textbf{CRF 40} & \\
			& \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed} & \textbf{CRF 23} & \textbf{Re-compressed}\\
			Luma~\citethis & 0.97 & 0.97 & 0.95 & 0.97 & 0.97 & 0.98 & 0.86 & 0.96 & 0.70 & 0.93\\
			CogVideo~\citethis & 0.96 & 0.98 & 0.92 & 0.97 & 0.98 & 0.98 & 0.82 & 0.98 & 0.67 & 0.95\\
			Vid.Crafter~\citethis & 0.95 & 0.98 & 0.94 & 0.96 & 0.98 & 0.99 & 0.85 & 0.98 & 0.69 & 0.95\\
			SVD~\citethis & 0.96 & 0.97 & 0.94 & 0.97 & 0.98 & 0.98 & 0.88 & 0.98 & 0.70 & 0.98
		\end{tblr}
	}
\end{table*}

==> tables/table1_v2.tex <==
% \usepackage{tabularray}
\begin{table}
	\centering
	\caption{Networks trained on synthetic images and tested on synthetic video frames}
	\label{tab:table_forsynth_im_noncompressed}
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{20mm}m{22mm}m{20mm}m{20mm}m{20mm}m{20mm}m{20mm}m{20mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{3} = {c=5}{0.634\linewidth,c},
				vline{1-3, 7-8} = {-}{},
				hline{1-3,7} = {-}{},
			}
			\textbf{Method} & \textbf{Images (AUC) } & \textbf{Videos (AUC)} &  &  &  & \\
			& \textbf{Baseline } & \textbf{Luma} & \textbf{CogVideo} & \textbf{VideoCrafter} & {\textbf{Stable Video}\\\textbf{Diffusion}} & {\textbf{Average }\\~}\\
			ResNet-34 & 0.983 & 0.576 & 0.623 & 0.616 & \textbf{0.647} & 0.615\\
			VGG-16 & 0.990 & 0.635 & 0.652 & \textbf{0.684} & 0.669 & \textbf{0.660}\\
			Xception & 0.996 & 0.592 & 0.638 & \textbf{0.670} & 0.664 & 0.641\\
			DenseNet & 0.975 & 0.559 & 0.584 & 0.647 & \textbf{0.678} & 0.624\\
			ResNet- 50(pre-trained) & 0.974 & 0.583 & \textbf{0.704} & 0.590 & 0.682 & 0.640\\
			DIF(pre-trained) & 0.992 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500\\
			Swin-T(pre-trained)& 0.891 & 0.652 & 0.694 & \textbf{0.728} & 0.719 & 0.698\\
			ResNet- 50(re-trained) & 0.946 & 0.572 & \textbf{0.736} & 0.604 & 0.710 & 0.656\\
			DIF(re-trained) & 0. & 0. & 0. & 0. & 0. & 0.\\
			Swin-T(re-trained)& 0. & 0. & 0. & \textbf{0.} & 0. & 0.\\
		\end{tblr}
	}
\end{table}

==> tables/table2_v2.tex <==
\begin{table}[!t]
	\centering
	\caption{Detection performance of existing synthetic image detectors that were retrained on H.264-compressed synthetic images on different synthetic video generation methods (Luma~\citethis, CogVideo~\citethis, Vid.Crafter~\citethis, and SVD~\citethis). Performance numbers are measured using AUC.}
	\label{tab:your_table_label}
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{30mm}m{12mm}m{9mm}m{14mm}m{16mm}m{9mm}m{12mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{3} = {c=5}{0.634\linewidth,c},
				vline{1-3, 7-8} = {-}{},
				hline{1-3, 6, 9} = {-}{},
			}
			\textbf{Method} & \textbf{Images} & \textbf{Videos} &  &  &  & \\
			& \textbf{Baseline} & \textbf{Luma} & \textbf{CogVideo} & \textbf{Vid.Crafter} & \textbf{SVD} & \textbf{Average}\\
			ResNet-34(R) ~\citethis & 0.989 & 0.663 & 0.687 & 0.700 & \textbf{0.727} & 0.694 \\
			VGG-16 (R)~\citethis & 0.993 & 0.719 & 0.743 & \textbf{0.754} & 0.729 & \textbf{0.736} \\
			Xception (R)~\citethis & 0.979 & 0.642 & 0.692 & \textbf{0.734} & 0.708 & 0.694 \\
			ResNet-50(R) ~\citethis & 0.963 & 0.604 & \textbf{0.770} & 0.646 & 0.738 & 0.689 \\
			DIF(R) ~\citethis & 0.994 & 0.617 & 0.634 & \textbf{0.655} & 0.624 & 0.632 \\
			Swin-T(R) ~\citethis & 0.948 & 0.679 & 0.730 & \textbf{0.758} & 0.742 & 0.727 \\
		\end{tblr}
	}
\end{table}

==> tables/table_1.tex <==
\begin{table}[!t]
	\centering
	\caption{Patch-level detection performance of existing synthetic image detectors that were trained or pretrained on synthetic images on different synthetic video generation methods (Luma~\citethis, CogVideo~\citethis, Vid.Crafter~\citethis, and SVD~\citethis). Performance numbers are measured using AUC. (P) denotes a pretrained version and (R) denotes and retrained version of a method.}
	\label{tab:table_forsynth_im_noncompressed}
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{30mm}m{12mm}m{9mm}m{14mm}m{16mm}m{9mm}m{12mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{3} = {c=5}{0.634\linewidth,c},
				vline{1-3, 7-8} = {-}{},
				hline{1-3, 6, 13} = {-}{},
			}
			\textbf{Method} & \textbf{Images} & \textbf{Videos} &  &  &  & \\
			& \textbf{Baseline} & \textbf{Luma} & \textbf{CogVideo} & \textbf{Vid.Crafter} & \textbf{SVD} & \textbf{Average}\\
			ResNet-50 (P)~\citethis & 0.974 & 0.583 & \textbf{0.704} & 0.590 & 0.682 & 0.640 \\
			DIF (P)~\citethis & 0.992 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 \\
			Swin-T (P)~\citethis & 0.891 & 0.652 & 0.694 & \textbf{0.728} & 0.719 & \textbf{0.698} \\
			ResNet-50 (R)~\citethis & 0.946 & 0.572 & \textbf{0.736} & 0.604 & 0.710 & 0.656 \\
			DIF (R)~\citethis & 0.991 & 0.581 & 0.603 & \textbf{0.617} & 0.573 & 0.594 \\
			Swin-T (R)~\citethis & 0.911 & 0.638 & 0.685 & \textbf{0.698} & 0.692 & 0.678 \\
			ResNet-34(R) ~\citethis & 0.983 & 0.576 & 0.623 & 0.616 & \textbf{0.647} & 0.615 \\
			VGG-16(R) ~\citethis & 0.990 & 0.635 & 0.652 & \textbf{0.684} & 0.669 & {0.660} \\
			Xception(R) ~\citethis & 0.996 & 0.592 & 0.638 & \textbf{0.670} & 0.664 & 0.641 \\
			DenseNet(R) ~\citethis & 0.975 & 0.559 & 0.584 & 0.647 & \textbf{0.678} & 0.624 \\
		\end{tblr}
	}
\end{table}

==> tables/table_1_v0.tex <==
\begin{table}[!t]
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{32mm}m{12mm}m{9mm}m{14mm}m{10mm}m{8mm}m{12mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{3} = {c=5}{0.634\linewidth,c},
				vline{1-3, 7-8} = {-}{},
				hline{1-3, 6,9, 14} = {-}{},
			}
			\textbf{Method} & \textbf{Images} & \textbf{Videos} &  &  &  & \\
			& \textbf{Baseline} & \textbf{Luma} & \textbf{CogVideo} & \textbf{VC-v1} & \textbf{SVD} & \textbf{Average}\\
			Corvi et al. (P)~\citethis & 0.974 & 0.583 & 0.704 & 0.590 & 0.682 & 0.640 \\
			DIF (P)~\citethis & 0.992 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 \\
			Swin-T (P)~\citethis & 0.891 & 0.652 & 0.694 & 0.728 & 0.719 & 0.698 \\
			Corvi et al. (R)~\citethis & 0.946 & 0.572 & 0.736 & 0.604 & 0.710 & 0.656 \\
			DIF (R)~\citethis & 0.991 & 0.581 & 0.603 & 0.617 & 0.573 & 0.594 \\
			Swin-T (R)~\citethis & 0.911 & 0.638 & 0.685 & 0.698 & 0.692 & 0.678 \\
			ResNet-34 ~\citethis & 0.983 & 0.576 & 0.623 & 0.616 & 0.647 & 0.615 \\
			VGG-16 ~\citethis & 0.990 & 0.635 & 0.652 & 0.684 & 0.669 & {0.660} \\
			Xception ~\citethis & 0.996 & 0.592 & 0.638 & 0.670 & 0.664 & 0.641 \\
			DenseNet ~\citethis & 0.975 & 0.559 & 0.584 & 0.647 & 0.678 & 0.624 \\
            MISLnet ~\citethis & 0.983 & 0.626 & 0.718 & 0.710 & 0.707 & 0.690 \\
		\end{tblr}
	}
    \caption{Patch-level detection performance of existing synthetic image detectors that were trained or pretrained on synthetic images on different synthetic video generation methods: Luma~\citethis, CogVideo~\citethis, VideoCrafter (VC-v1)~\citethis, and Stable Video Diffusion (SVD)~\citethis. Performance numbers are measured using AUC. (P) denotes a pretrained version and (R) denotes and retrained version of a method.}
    \label{tab:synth_im_det_on_videos}
\end{table}

==> tables/table_2.tex <==
\begin{table}[!t]
	\centering
	\caption{Patch-level detection performance of existing synthetic image detectors that were retrained on H.264-compressed synthetic images on different synthetic video generation methods (Luma~\citethis, CogVideo~\citethis, Vid.Crafter~\citethis, and SVD~\citethis). Performance numbers are measured using AUC. (P) denotes a pretrained version and (R) denotes and retrained version of a method.}
	\label{tab:your_table_label}
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{30mm}m{12mm}m{9mm}m{14mm}m{16mm}m{9mm}m{12mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{3} = {c=5}{0.634\linewidth,c},
				vline{1-3, 7-8} = {-}{},
				hline{1-3, 6, 13} = {-}{},
			}
			\textbf{Method} & \textbf{Images} & \textbf{Videos} &  &  &  & \\
			& \textbf{Baseline} & \textbf{Luma} & \textbf{CogVideo} & \textbf{Vid.Crafter} & \textbf{SVD} & \textbf{Average}\\
			ResNet-50 (P)~\citethis & 0.974 & 0.583 & \textbf{0.704} & 0.590 & 0.682 & 0.640 \\
			DIF (P)~\citethis & 0.992 & 0.500 & 0.500 & 0.500 & 0.500 & 0.500 \\
			Swin-T (P)~\citethis & 0.891 & 0.652 & 0.694 & \textbf{0.728} & 0.719 & \textbf{0.698} \\
			ResNet-50 (R)~\citethis & 0.963 & 0.604 & 0.770 & 0.646 & 0.738 & 0.689 \\
			DIF (R)~\citethis & 0.994 & \ldash & \ldash & \ldash & \ldash & \ldash \\
			Swin-T (R)~\citethis & 0.948 & \ldash & \ldash & \ldash & \ldash & \ldash \\
			ResNet-34 (R)~\citethis & 0.989 & 0.663 & 0.687 & 0.700 & \textbf{0.727} & 0.694 \\
			VGG-16 (R)~\citethis & 0.993 & 0.719 & 0.743 & \textbf{0.754} & 0.729 & \textbf{0.736} \\
			Xception (R)~\citethis & 0.979 & 0.642 & 0.692 & \textbf{0.734} & 0.708 & 0.694 \\
			DenseNet(R) ~\citethis & \ldash & \ldash & \ldash & \ldash & \ldash & \ldash \\
		\end{tblr}
	}
\end{table}

==> tables/table_2_v0.tex <==
\begin{table}[!t]
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{32mm}m{12mm}m{9mm}m{14mm}m{10mm}m{8mm}m{12mm}m{14mm}},
				row{1-2} = {c},
				column{2-9} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{3} = {c=6}{0.634\linewidth,c},
				vline{1-3, 7-9} = {-}{},
				hline{1-3,6, 11} = {-}{},
			}
			\textbf{Method} & \textbf{Images} & \textbf{Videos} &  &  &  & \\
			& \textbf{Baseline} & \textbf{Luma} & \textbf{CogVideo} & \textbf{VC-v1} & \textbf{SVD} & \textbf{Average}& {\textbf{Vs.}\\\textbf{no H.264}}\\
			Corvi et al.(R)~\citethis & 0.963 & 0.604 & 0.770 & 0.646 & 0.738 & 0.689 & +0.033 \\
			DIF(R)~\citethis & 0.994 & 0.617 & 0.634 & 0.655 & 0.624 & 0.632 & +0.038 \\
			Swin-T(R)~\citethis & 0.948 & 0.679 & 0.730 & 0.758 & 0.742 & 0.727& +0.049 \\
            ResNet-34~\citethis & 0.989 & 0.663 & 0.687 & 0.700 & 0.727 & 0.694 & +0.079 \\
            VGG-16~\citethis & 0.993 & 0.719 & 0.743 & 0.754 & 0.729 & 0.736 & +0.076 \\
            Xception~\citethis & 0.979 & 0.642 & 0.692 & 0.734 & 0.708 & 0.694 & +0.053 \\
            DenseNet ~\citethis & 0.980 & 0.604 & 0.628 & 0.691 & 0.703 & 0.656 & +0.032 \\
            MISLnet ~\citethis & 0.995 & 0.674 & 0.759 & 0.784 & 0.760 & 0.744 & +0.054 \\
		\end{tblr}
	}
    \caption{Patch-level detection performance of existing synthetic image detectors that were retrained on H.264-compressed synthetic images on different synthetic video generation methods: Luma~\citethis, CogVideo~\citethis, VideoCrafter (VC-v1)~\citethis, and Stable Video Diffusion (SVD)~\citethis). (R) signifies the retraining of the detectors. Performance numbers are measured using AUC.}
    \label{tab:synth_im_det_on_videos_h264}
\end{table}

==> tables/table_3.tex <==
\begin{table}[!t]
	\centering
	\resizebox{0.8\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {Q[215]Q[333]Q[346]},
				column{2} = {c},
				column{3} = {c},
				vlines,
				hline{1-2,10} = {-}{},
			}
			 \textbf{Architecture} & \textbf{Average AUC}\\
              Corvi et al. & 0.944\\
              DIF & 0.961\\
              Swin-T & 0.979\\
              ResNet-34 & 0.937\\
              VGG-16 & 0.950\\
              Xception & 0.955\\
              DenseNet &0 .947 \\
			 MISLnet & \textbf{0.982}\\
		\end{tblr}
	}
    \caption{Average patch-level detection performance of different methods with different underlying network architectures on the set of testing videos gathered from all synthetic video generators used in this paper. These include: Luma~\citethis, CogVideo~\citethis, VideoCrafter~\citethis, and Stable Video Diffusion~\citethis. Performance numbers are measured using AUC.}
    \label{tab:exp1_synth_vid_det}
\end{table}

==> tables/table_few_shot.tex <==
\begin{table}[!h]
	\centering
	\resizebox{0.8\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{35mm}m{18mm}},
				column{2,3} = {c},
				vlines,
				hline{1-2,5} = {-}{},
			}
			\textbf{Generation Method} & \textbf{Zero-Shot} & \textbf{Few-Shot} & \textbf{RER}\\
            Sora~\cite{sora} & 0.530 & 0.982 & 96.2\%\\
			Pika~\cite{Pika} & 0.620 & 0.989 & 97.1\%\\
			VideoCrafter v2~\cite{videocrafter2} & 0.939 & 0.996 & 93.4\%
		\end{tblr}
	}
    \caption{Zero-Shot and Few-Shot detection performance of MISLnet~\cite{openset}, which was trained on the training portion of our synthetic video dataset, and tested on new video generation sources: VideoCrafter v2~\cite{videocrafter2}, SORA~\cite{sora}, Pika~\cite{Pika}. Performance numbers are measured using AUC. Relative Error Reduction shown as RER}
    \label{tab:few_shot_learning}
\end{table}
   
   
   
   


==> tables/tables_one_out.tex <==
\begin{table}[!t]
	\centering
	\caption{The Evaluation of Transferability of MISLnet\citethis trained on a portion of the videos gathered from synthetic video generators used in this paper to videos unseen by the detector. These include: Luma~\citethis, CogVideo~\citethis, VideoCrafter~\citethis, Stable Video Diffusion~\citethis,SORA\citethis,Pika\citethis. The F noted to the right side of some rows signifies that the test results are from the fine-tuned version. Performance numbers are measured using AUC.}
	\resizebox{0.8\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {Q[396]Q[333]Q[346]},
				column{2} = {c},
				column{3} = {c},
				vlines,
				hline{1-2,9,12} = {-}{},
			}
			\textbf{Test Generator} & \textbf{Baseline AUC} & \textbf{Test AUC}\\
			VideoCrafter v1\citethis & 0.993 & 0.773\\
			Cogvideo\citethis & 0.990 & 0.671\\
			Luma\citethis & 0.991 & 0.702\\
			SVD\citethis & 0.985 & 0.760\\
			SORA\citethis & 0.998 & 0.530\\
			Pika\citethis & 0.998 & 0.620\\
			VideoCrafter v2\citethis & 0.998 & \textbf{0.939}\\
			SORA(F)\citethis & 0.998 & 0.982\\
			Pika(F)\citethis & 0.998 & 0.989\\
			VideoCrafter v2(F)\citethis & 0.998 & \textbf{0.996}
		\end{tblr}
	}
\end{table}

==> tables/video_dataset_stats_v0.tex <==
\definecolor{Mercury}{rgb}{0.913,0.913,0.913}
\begin{table}
    \centering
    \resizebox{\linewidth}{!}{%
    \begin{tblr}{
      width = \linewidth,
      colspec = {m{3mm}m{28mm}m{13mm}m{14mm}m{13mm}m{14mm}m{13mm}m{14mm}},
      row{1,2} = {c},
      column{3-8} = {c},
      column{2} = {l},
      row{5, 10} = {Mercury},
      cell{1}{1} = {r=2}{},
      cell{1}{2} = {r=2}{},
      cell{1}{3} = {c=2}{0.244\linewidth},
      cell{1}{5} = {c=2}{0.244\linewidth},
      cell{1}{7} = {c=2}{0.244\linewidth},
      cell{3}{1} = {r=2}{c},
      cell{5}{1} = {c=2}{0.192\linewidth},
      cell{6}{1} = {r=4}{c},
      cell{10}{1} = {c=2}{0.192\linewidth},
      vline{1,9} = {-}{},
      vline{2-3,5,7} = {1-4,5-10}{},
      hline{1,3,5-6,10-11} = {-}{},
      hline{2} = {3-8}{},
    }
        & \textbf{Dataset} & \textbf{Training} &  & \textbf{Validation} &  & \textbf{Testing} & \\
        &  & \textbf{\# Videos} & \textbf{\# Frames} & \textbf{\# Videos} & \textbf{\# Frames} & \textbf{\# Videos} & \textbf{\# Frames}\\
        \begin{sideways}\textbf{Real}\end{sideways}
        & MIT~\citethis & 3,991  & 119,740  & 377 & 11,300 & 945 & 28,357 \\
        & Video-ACID~\citethis & 3,663  & 109,875 & 407 & 12,208 & 716 & 21,649 \\
        \textbf{Total} &  & 7,654 & 229,615 & 784 & 23,508 & 1,661 & 50,006 \\
        
        \begin{sideways}\textbf{Synthetic}\end{sideways}
        & Luma~\citethis & 1,423 & 42,708 & 158 & 4,746 & 412 & 12,380 \\
        & VideoCrafter~\citethis & 2,220 & 66,603 & 247 & 7,400 & 618 & 18,540 \\
        & CogVideo~\citethis & 4,527 & 135,812 & 503 & 15,090 & 1,258 & 37,726 \\
        & SVD~\citethis & 1,735 & 52,056 & 193 & 5,784 & 482 & 14,460\\
        \textbf{Total} &  & 9,905 & 297,179 & 1,101 & 33,020 & 2,770 & 83,106  
    \end{tblr}
    }
    \caption{Dataset statistics for training and evaluating detection systems on synthetic video data.}
    \label{tab:video_dataset_stats}
\end{table}

==> tables/video_generator_table.tex <==
\begin{table}[!t]
	\centering
	\resizebox{\linewidth}{!}{%
		\begin{tblr}{
				width = \linewidth,
				colspec = {m{32mm}m{12mm}m{16mm}m{14mm}m{9mm}m{14mm}},
				row{1-2} = {c},
				column{2-8} = {c},
				column{1} = {l},
				cell{1}{1} = {r=2}{},
				cell{1}{2} = {c=5}{0.634\linewidth,c},
				vline{1-2, 6, 7} = {-}{},
				hline{1-3,6, 11} = {-}{},
			}
			\textbf{Method}   & \textbf{Videos} &  &  &  & \\
			  & \textbf{Luma} & \textbf{CogVideo} & \textbf{VC-v1} & \textbf{SVD} & \textbf{Average}\\
			Corvi et al.(R)~\citethis  & 0.921 & \textbf{0.935} & 0.940 & 0.939 & 0.934 \\
			DIF(R)~\citethis  & 0.938 & 0.957 & 0.969 & 0.973 & 0.959 \\
			Swin-T(R)~\citethis  & 0.960 & 0.964 & 0.986 & 0.991 & 0.975 \\
            ResNet-34~\citethis  & 0.916 & 0.930 & 0.942 & 0.951 & 0.935  \\
            VGG-16~\citethis  & 0.937 & 0.944 & 0.965 & 0.960 & 0.951  \\
            Xception~\citethis  & 0.928 & 0.951 & 0.973 & 0.969 & 0.955  \\
            DenseNet ~\citethis  & 0.918 & 0.924 & 0.964 & 0.968 & 0.943  \\
            MISLnet ~\citethis  & \textbf{0.975} & \textbf{0.980} & \textbf{0.991} & \textbf{0.987} & \textbf{0.983}  \\
		\end{tblr}
	}
    \caption{Patch-level detection performance of methods trained and tested on different synthetic video generation methods: Luma~\citethis, CogVideo~\citethis, VideoCrafter (VC-v1)~\citethis, and Stable Video Diffusion (SVD)~\citethis. Performance numbers are measured using AUC.}
    \label{tab:exp1_synth_vid_det}
\end{table}
